A Multi-State Diagnosis and Prognosis Framework with Feature Learning for Tool Condition Monitoring

In this paper, a multi-state diagnosis and prognosis (MDP) framework is proposed for tool condition monitoring via a deep belief network based multi-state approach (DBNMS). For fault diagnosis, a cost-sensitive deep belief network (namely ECS-DBN) is applied to deal with the imbalanced data problem for tool state estimation. An appropriate prognostic degradation model is then applied for tool wear estimation based on the different tool states. The proposed framework has the advantage of automatic feature representation learning and shows better performance in accuracy and robustness. The effectiveness of the proposed DBNMS is validated using a real-world dataset obtained from the gun drilling process. This dataset contains a large amount of measured signals involving different tool geometries under various operating conditions. The DBNMS is examined for both the tool state estimation and tool wear estimation tasks. In the experimental studies, the prediction results are evaluated and compared with popular machine learning approaches, which show the superior performance of the proposed DBNMS approach.

==> table/experimental_conditions.tex <==
\begin{table}[t]
	\centering
	%\vspace{-0.2cm}
	\caption{Detailed real-world high aspect ratio deep hole gun drilling experimental conditions include tool diameter, spindle speed, feed rate and machining time for 20 drilling inserts with 6 different tool geometries.}
	%\vspace{-0.2cm}
	\label{experimental_conditions}
	\begin{scriptsize}
	\resizebox{\columnwidth}{!}{
		\begin{tabular}{c|c|c|c|c|c|c}
			\hline
			\begin{tabular}[c]{@{}c@{}}Hole\\Index\end{tabular} & \begin{tabular}[c]{@{}c@{}}Drill\\Depth\\(mm)\end{tabular} & Tool Geometry                   & \begin{tabular}[c]{@{}c@{}}Tool\\Diameter\\(mm)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Spindle\\Speed\\(rpm)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Feed\\Rate\\($\mu m$/rev)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Machining\\Time(s)\end{tabular} \\ \hline
			H1\_01     & 50                                                          & \multirow{2}{*}{1450mm\_N4\_R9} & 8.05                                                          & 1200                                                           & 20                                                            & 125.00                                                                 \\ \cline{1-2} \cline{4-7} 
			H1\_02     & 50                                                          &                                 & 8.05                                                          & 1200                                                           & 20                                                            & 125.00                                                                   \\ \hline
			H2\_01     & 50                                                          & 1450mm\_N4\_R1                  & 8.05                                                          & 800                                                            & 20                                                            & 187.50                                                                 \\ \hline
			H2\_02     & 50                                                          & 1450mm\_N4\_R1                  & 8.05                                                          & 800                                                            & 20                                                            & 187.50                                                                   \\ \hline
			H2\_03     & 50                                                          & 1650mm\_N8\_R1                  & 8.02                                                          & 1650                                                           & 16                                                            & 113.64                                                                     \\ \hline
			H3\_01     & 50                                                          & \multirow{3}{*}{1450mm\_N8\_R9} & 8.05                                                          & 1650                                                           & 16                                                            & 113.64                                                                     \\ \cline{1-2} \cline{4-7} 
			H3\_02     & 50                                                          &                                 & 8.05                                                          & 1650                                                           & 16                                                            & 113.64                                                                   \\ \cline{1-2} \cline{4-7} 
			H3\_03     & 50                                                          &                                 & 8.05                                                          & 1650                                                           & 16                                                            & 113.64                                                                   \\ \hline
			H3\_04     & 50                                                          & \multirow{2}{*}{1450mm\_N8\_R9} & 8.05                                                          & 1650                                                           & 16                                                            & 113.64                                                             \\ \cline{1-2} \cline{4-7} 
			H3\_05     & 50                                                          &                                 & 8.05                                                          & 1650                                                           & 16                                                            & 113.64                                                              \\ \hline
			H3\_06     & 50                                                          & \multirow{2}{*}{1650mm\_N8\_R9} & 8.02                                                          & 1650                                                           & 16                                                            & 113.64                                                                \\ \cline{1-2} \cline{4-7} 
			H3\_07     & 50                                                          &                                 & 8.02                                                          & 1650                                                           & 16                                                            & 113.64                                                                \\ \hline
			H3\_08     & 50                                                          & \multirow{2}{*}{1650mm\_N8\_R9} & 8.02                                                          & 1650                                                           & 16                                                            & 113.64                                                                 \\ \cline{1-2} \cline{4-7} 
			H3\_09     & 50                                                          &                                 & 8.02                                                          & 1650                                                           & 16                                                            & 113.64                                                               \\ \hline
			H3\_10     & 50                                                          & 1650mm\_N8\_R1                  & 8.02                                                          & 1650                                                           & 16                                                            & 113.64                                                              \\ \hline
			H4\_01     & 50                                                          & \multirow{3}{*}{1219mm\_N8\_R9} & 8.08                                                          & 1650                                                           & 16                                                            & 113.64                                                                     \\ \cline{1-2} \cline{4-7} 
			H4\_02     & 50                                                          &                                 & 8.08                                                          & 1650                                                           & 16                                                            & 113.64                                                                 \\ \cline{1-2} \cline{4-7} 
			H4\_03     & 50                                                          &                                 & 8.08                                                          & 1650                                                           & 16                                                            & 113.64                                                                  \\ \hline
			H5\_01     & 50                                                          & 1450mm\_N8\_R9                  & 8.045                                                         & 1650                                                           & 16                                                            & 113.64                                                              \\ \hline
			H5\_02     & 50                                                          & 1450mm\_N8\_R9                  & 8.045                                                         & 1650                                                           & 16                                                            & 113.64                                                           \\ \hline
		\end{tabular}
		}
		%\vspace{-0.5cm}
	\end{scriptsize}
	\vspace{-0.4cm}
\end{table}

\iffalse
\begin{table}[t]
	\centering
	\vspace{-0.2cm}
	\caption{\scriptsize Experimental Conditions}
	\vspace{-0.2cm}
	\label{experimental_conditions}
	\begin{tiny}
		\begin{tabular}{|c|c|c|c|c|c|c|c|}
			\hline
			\begin{tabular}[c]{@{}c@{}}Hole\\Index\end{tabular} & \begin{tabular}[c]{@{}c@{}}Drill\\Depth\\(mm)\end{tabular} & Tool Geometry                   & \begin{tabular}[c]{@{}c@{}}Tool\\Diameter\\(mm)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Spindle\\Speed\\ (rpm)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Feed\\Rate\\(um/rev)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Machining\\ Time (s)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Tool\\Final\\State\end{tabular} \\ \hline
			H1\_01     & 50                                                          & \multirow{2}{*}{1450mm\_N4\_R9} & 8.05                                                          & 1200                                                           & 20                                                            & 125.00                                                        & Chipping         \\ \cline{1-2} \cline{4-8} 
			H1\_02     & 50                                                          &                                 & 8.05                                                          & 1200                                                           & 20                                                            & 125.00                                                        & Broken           \\ \hline
			H2\_01     & 50                                                          & 1450mm\_N4\_R1                  & 8.05                                                          & 800                                                            & 20                                                            & 187.50                                                        & Chipping         \\ \hline
			H2\_02     & 50                                                          & 1450mm\_N4\_R1                  & 8.05                                                          & 800                                                            & 20                                                            & 187.50                                                        & Broken           \\ \hline
			H2\_03     & 50                                                          & 1650mm\_N8\_R1                  & 8.02                                                          & 1650                                                           & 16                                                            & 113.64                                                        & Worn             \\ \hline
			H3\_01     & 50                                                          & \multirow{3}{*}{1450mm\_N8\_R9} & 8.05                                                          & 1650                                                           & 16                                                            & 113.64                                                        & Worn             \\ \cline{1-2} \cline{4-8} 
			H3\_02     & 50                                                          &                                 & 8.05                                                          & 1650                                                           & 16                                                            & 113.64                                                        & Worn             \\ \cline{1-2} \cline{4-8} 
			H3\_03     & 50                                                          &                                 & 8.05                                                          & 1650                                                           & 16                                                            & 113.64                                                        & Worn             \\ \hline
			H3\_04     & 50                                                          & \multirow{2}{*}{1450mm\_N8\_R9} & 8.05                                                          & 1650                                                           & 16                                                            & 113.64                                                        & Chipping         \\ \cline{1-2} \cline{4-8} 
			H3\_05     & 50                                                          &                                 & 8.05                                                          & 1650                                                           & 16                                                            & 113.64                                                        & Chipping         \\ \hline
			H3\_06     & 50                                                          & \multirow{2}{*}{1650mm\_N8\_R9} & 8.02                                                          & 1650                                                           & 16                                                            & 113.64                                                        & Worn             \\ \cline{1-2} \cline{4-8} 
			H3\_07     & 50                                                          &                                 & 8.02                                                          & 1650                                                           & 16                                                            & 113.64                                                        & Worn             \\ \hline
			H3\_08     & 50                                                          & \multirow{2}{*}{1650mm\_N8\_R9} & 8.02                                                          & 1650                                                           & 16                                                            & 113.64                                                        & Worn             \\ \cline{1-2} \cline{4-8} 
			H3\_09     & 50                                                          &                                 & 8.02                                                          & 1650                                                           & 16                                                            & 113.64                                                        & Worn             \\ \hline
			H3\_10     & 50                                                          & 1650mm\_N8\_R1                  & 8.02                                                          & 1650                                                           & 16                                                            & 113.64                                                        & Chipping         \\ \hline
			H4\_01     & 50                                                          & \multirow{3}{*}{1219mm\_N8\_R9} & 8.08                                                          & 1650                                                           & 16                                                            & 113.64                                                        & Worn             \\ \cline{1-2} \cline{4-8} 
			H4\_02     & 50                                                          &                                 & 8.08                                                          & 1650                                                           & 16                                                            & 113.64                                                        & Worn             \\ \cline{1-2} \cline{4-8} 
			H4\_03     & 50                                                          &                                 & 8.08                                                          & 1650                                                           & 16                                                            & 113.64                                                        & Broken           \\ \hline
			H5\_01     & 50                                                          & 1450mm\_N8\_R9                  & 8.045                                                         & 1650                                                           & 16                                                            & 113.64                                                        & Chipping         \\ \hline
			H5\_02     & 50                                                          & 1450mm\_N8\_R9                  & 8.045                                                         & 1650                                                           & 16                                                            & 113.64                                                        & Chipping         \\ \hline
		\end{tabular}
		%\vspace{-0.5cm}
	\end{tiny}
\end{table}

\fi


\iffalse
\begin{table*}[!t]
	\centering
	\caption{Experimental Conditions}
	\label{experimental_conditions}
	\begin{scriptsize}
	\begin{tabular}{|c|c|c|c|c|c|c|c|}
		\hline
		Hole Index & \begin{tabular}[c]{@{}c@{}}Drill Depth \\ (mm)\end{tabular} & Tool Geometry                   & \begin{tabular}[c]{@{}c@{}}Tool Diameter \\ (mm)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Spindle Speed \\ (rpm)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Feed Rate \\ (um/rev)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Machining \\ Time (s)\end{tabular} & Tool Final State \\ \hline
		H1\_01     & 50                                                          & \multirow{2}{*}{1450mm\_N4\_R9} & 8.05                                                          & 1200                                                           & 20                                                            & 125.00                                                        & Chipping         \\ \cline{1-2} \cline{4-8} 
		H1\_02     & 50                                                          &                                 & 8.05                                                          & 1200                                                           & 20                                                            & 125.00                                                        & Broken           \\ \hline
		H2\_01     & 50                                                          & 1450mm\_N4\_R1                  & 8.05                                                          & 800                                                            & 20                                                            & 187.50                                                        & Chipping         \\ \hline
		H2\_02     & 50                                                          & 1450mm\_N4\_R1                  & 8.05                                                          & 800                                                            & 20                                                            & 187.50                                                        & Broken           \\ \hline
		H2\_03     & 50                                                          & 1650mm\_N8\_R1                  & 8.02                                                          & 1650                                                           & 16                                                            & 113.64                                                        & Worn             \\ \hline
		H3\_01     & 50                                                          & \multirow{3}{*}{1450mm\_N8\_R9} & 8.05                                                          & 1650                                                           & 16                                                            & 113.64                                                        & Worn             \\ \cline{1-2} \cline{4-8} 
		H3\_02     & 50                                                          &                                 & 8.05                                                          & 1650                                                           & 16                                                            & 113.64                                                        & Worn             \\ \cline{1-2} \cline{4-8} 
		H3\_03     & 50                                                          &                                 & 8.05                                                          & 1650                                                           & 16                                                            & 113.64                                                        & Worn             \\ \hline
		H3\_04     & 50                                                          & \multirow{2}{*}{1450mm\_N8\_R9} & 8.05                                                          & 1650                                                           & 16                                                            & 113.64                                                        & Chipping         \\ \cline{1-2} \cline{4-8} 
		H3\_05     & 50                                                          &                                 & 8.05                                                          & 1650                                                           & 16                                                            & 113.64                                                        & Chipping         \\ \hline
		H3\_06     & 50                                                          & \multirow{2}{*}{1650mm\_N8\_R9} & 8.02                                                          & 1650                                                           & 16                                                            & 113.64                                                        & Worn             \\ \cline{1-2} \cline{4-8} 
		H3\_07     & 50                                                          &                                 & 8.02                                                          & 1650                                                           & 16                                                            & 113.64                                                        & Worn             \\ \hline
		H3\_08     & 50                                                          & \multirow{2}{*}{1650mm\_N8\_R9} & 8.02                                                          & 1650                                                           & 16                                                            & 113.64                                                        & Worn             \\ \cline{1-2} \cline{4-8} 
		H3\_09     & 50                                                          &                                 & 8.02                                                          & 1650                                                           & 16                                                            & 113.64                                                        & Worn             \\ \hline
		H3\_10     & 50                                                          & 1650mm\_N8\_R1                  & 8.02                                                          & 1650                                                           & 16                                                            & 113.64                                                        & Chipping         \\ \hline
		H4\_01     & 50                                                          & \multirow{3}{*}{1219mm\_N8\_R9} & 8.08                                                          & 1650                                                           & 16                                                            & 113.64                                                        & Worn             \\ \cline{1-2} \cline{4-8} 
		H4\_02     & 50                                                          &                                 & 8.08                                                          & 1650                                                           & 16                                                            & 113.64                                                        & Worn             \\ \cline{1-2} \cline{4-8} 
		H4\_03     & 50                                                          &                                 & 8.08                                                          & 1650                                                           & 16                                                            & 113.64                                                        & Broken           \\ \hline
		H5\_01     & 50                                                          & 1450mm\_N8\_R9                  & 8.045                                                         & 1650                                                           & 16                                                            & 113.64                                                        & Chipping         \\ \hline
		H5\_02     & 50                                                          & 1450mm\_N8\_R9                  & 8.045                                                         & 1650                                                           & 16                                                            & 113.64                                                        & Chipping         \\ \hline
	\end{tabular}
	\end{scriptsize}
\end{table*}
\fi

==> table/gun_drilling_dataset_details.tex <==
\begin{table}[!t]
\centering
\caption{Detailed number of data samples and imbalance ratio of the imbalanced gun drilling dataset.}
\label{tab:gun_drilling_dataset_description}
%\begin{scriptsize}
\begin{tabular}{ll}
\hline
\hline
Number of Signal Channels    & 14       \\ %\hline
Total Number of Data Samples & 19,712,414 \\ %\hline
Number of Training Samples   & 13,798,690 \\ %\hline
Number of Testing Samples    & 5,913,724  \\ 
%Imbalance Ratio & 10 \\\hline
\end{tabular}
%\end{scriptsize}
\end{table}

==> table/gun_drilling_dataset_results_ranking_matrix.tex <==
\iffalse
\begin{table*}[t]
\centering
\caption{Average Ranks of Different Methods on Imbalanced Gun Drilling Dataset}
\label{tab:gundrilling_results_ranking_matrix}
\begin{tiny}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
Model Name      & ECSDBN       & CSDBN & \begin{tabular}[c]{@{}c@{}}SMOTE-SVM\\ -DBN\end{tabular} & \begin{tabular}[c]{@{}c@{}}ADASYN\\ -DBN\end{tabular} & \begin{tabular}[c]{@{}c@{}}SMOTE-borderline2\\ -DBN\end{tabular} & \begin{tabular}[c]{@{}c@{}}SMOTE-borderline1\\ -DBN\end{tabular} & \begin{tabular}[c]{@{}c@{}}SMOTE\\ -DBN\end{tabular} & DBN           \\ \hline
Average Ranks & \textbf{2.2} & 3.9   & 3.2                                                      & 2.8                                                              & 3.8                                                              & 6.4                                                              & 5.7                                                  & 8             \\ \hline
Model Name      & SVM          & MLP   & KNeighborsClassifier                                     & GradientBoostingClassifier                                       & LogisticRegression                                               & AdaBoostClassifier                                               & Lasso                                                & SGDClassifier \\ \hline
Average Ranks & 9            & 11.2  & 11.4                                                     & 10.4                                                             & 13.8                                                             & 14.8                                                             & 13.4                                                 & 16            \\ \hline
\end{tabular}
\end{tiny}
\end{table*}
\fi

\begin{table*}[t]
\centering
\caption{Average Ranks of Different Methods on Imbalanced Gun Drilling Dataset}
\label{tab:gundrilling_results_ranking_matrix_withoutROC}
\begin{tiny}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
Model Name      & ECSDBN       & CSDBN & \begin{tabular}[c]{@{}c@{}}SMOTE-SVM\\ -DBN\end{tabular} & \begin{tabular}[c]{@{}c@{}}ADASYN\\ -DBN\end{tabular} & \begin{tabular}[c]{@{}c@{}}SMOTE-borderline2\\ -DBN\end{tabular} & \begin{tabular}[c]{@{}c@{}}SMOTE-borderline1\\ -DBN\end{tabular} & \begin{tabular}[c]{@{}c@{}}SMOTE\\ -DBN\end{tabular} & DBN           \\ \hline
Average Ranks & \textbf{2.5} & 4.375 & 3.25  & 2.5  & 3.5   & 6.375 & 5.5  & 8  \\ \hline            
Model Name      & SVM          & MLP   & KNeighborsClassifier                                     & GradientBoostingClassifier                                       & LogisticRegression                                               & AdaBoostClassifier                                               & Lasso                                                & SGDClassifier \\ \hline
Average Ranks & 9            & 11.25 & 11.25 & 10.5 & 13.75 & 14.75 & 13.5 & 16 \\ \hline
\end{tabular}
\end{tiny}
\end{table*}


==> table/gun_drilling_fault_diagnosis_simulation_results.tex <==
\iffalse
\begin{table*}[t]
\centering
\caption{Simulation results of different models on gun drilling dataset.}
\label{tab:fault_diagnosis_simulation_results_gundrilling}
%\begin{scriptsize}
\begin{tabular}{|c|c|c|c|c|c|}
	\hline \hline
	Model Name & ECSDBN                    & MLP              & Support Vector Machine          & K-Nearest Neighbors           & SGD Classifier          \\ \hline
	Accuracy   & \textbf{0.9955 $\pm$ 0.0012} & 0.9812 $\pm$ 0.0029    & 0.9049 $\pm$ 0.1097 & 0.9587 $\pm$ 0.0044 & 0.7935 $\pm$ 0.0582 \\ \hline
	G\_mean    & \textbf{0.9932 $\pm$ 0.0017} & 0.9822 $\pm$ 0.0033    & 0.8346 $\pm$ 0.2867 & 0.9570 $\pm$ 0.0036 & 0.7041 $\pm$ 0.1159 \\ \hline
	F1\_score  & \textbf{0.9955 $\pm$ 0.0012} & 0.9763 $\pm$ 0.0037    & 0.9049 $\pm$ 0.1097 & 0.9587 $\pm$ 0.0044 & 0.7935 $\pm$ 0.0582 \\ \hline \hline
	Model Name & Logistic Regression    & Gradient Boosting & Random Forest  & AdaBoost      & Lasso         \\ \hline
	Accuracy   & 0.8755 $\pm$ 0.0205          & 0.9261 $\pm$ 0.0986    & 0.9810 $\pm$ 0.0050 & 0.8410 $\pm$ 0.0637 & 0.7286 $\pm$ 0.1281 \\ \hline
	G\_mean    & 0.8529 $\pm$ 0.0324          & 0.8746 $\pm$ 0.2385    & 0.9782 $\pm$ 0.0060 & 0.7788 $\pm$ 0.1113 & 0.4229 $\pm$ 0.4066 \\ \hline
	F1\_score  & 0.8755 $\pm$ 0.0205          & 0.9261 $\pm$ 0.0986    & 0.9810 $\pm$ 0.0050 & 0.8410 $\pm$ 0.0637 & 0.7286 $\pm$ 0.1281 \\ \hline
\end{tabular}
%\end{scriptsize}
\end{table*}
\fi

\begin{table*}[t]
	\centering
	\caption{Compare the Performance of Different Algorithms on Gun Drilling Imbalanced Dataset In Terms of Accuracy, G\_Mean, ROC\_score, Precision}
	\label{tab:imbalance_binary_classification_results_gun_drilling}
	\begin{tabular}{|c|c|c|c|c|}
		\hline
		Model Name                 & Accuracy      & G\_mean       & ROC\_score    & Precision     \\ \hline
		ECSDBN                     & 0.9960 $\pm$ 0.0002 & \textbf{0.9946 $\pm$ 0.0011} & \textbf{0.9946 $\pm$ 0.0011} & \textbf{0.9996 $\pm$ 0.0002} \\ \hline
		CSDBN                      & 0.9957 $\pm$ 0.0012 & 0.9916 $\pm$ 0.0026 & 0.9916 $\pm$ 0.0025 & 0.9987 $\pm$ 0.0007 \\ \hline
		SMOTE-SVM-DBN              & 0.9961 $\pm$ 0.0003 & 0.9858 $\pm$ 0.0011 & 0.9859 $\pm$ 0.0011 & 0.9974 $\pm$ 0.0002 \\ \hline
		ADASYN-DBN                 & \textbf{0.9964 $\pm$ 0.0004} & 0.9857 $\pm$ 0.0016 & 0.9858 $\pm$ 0.0016 & 0.9973 $\pm$ 0.0003 \\ \hline
		SMOTE-borderline2-DBN      & 0.9962 $\pm$ 0.0001 & 0.9852 $\pm$ 0.0010 & 0.9853 $\pm$ 0.0010 & 0.9972 $\pm$ 0.0002 \\ \hline
		SMOTE-borderline1-DBN      & 0.9958 $\pm$ 0.0003 & 0.9837 $\pm$ 0.0021 & 0.9838 $\pm$ 0.0020 & 0.9969 $\pm$ 0.0004 \\ \hline
		SMOTE-DBN                  & 0.9959 $\pm$ 0.0001 & 0.9837 $\pm$ 0.0010 & 0.9838 $\pm$ 0.0010 & 0.9969 $\pm$ 0.0002 \\ \hline
		DBN                        & 0.9954 $\pm$ 0.0006 & 0.9830 $\pm$ 0.0027 & 0.9831 $\pm$ 0.0027 & 0.9968 $\pm$ 0.0005 \\ \hline
		SVM                        & 0.9894 $\pm$ 0.0283 & 0.8943 $\pm$ 0.3143 & 0.9443 $\pm$ 0.1562 & 0.9898 $\pm$ 0.0284 \\ \hline
		MLP                        & 0.9683 $\pm$ 0.0064 & 0.8492 $\pm$ 0.0350 & 0.8601 $\pm$ 0.0296 & 0.9733 $\pm$ 0.0056 \\ \hline
		KNeighborsClassifier       & 0.9733 $\pm$ 0.0026 & 0.8460 $\pm$ 0.0214 & 0.8579 $\pm$ 0.0181 & 0.9725 $\pm$ 0.0035 \\ \hline
		GradientBoostingClassifier & 0.9821 $\pm$ 0.0353 & 0.8088 $\pm$ 0.3910 & 0.9025 $\pm$ 0.1947 & 0.9822 $\pm$ 0.0354 \\ \hline
		LogisticRegression         & 0.9412 $\pm$ 0.0096 & 0.5903 $\pm$ 0.1058 & 0.6791 $\pm$ 0.0545 & 0.9398 $\pm$ 0.0095 \\ \hline
		AdaBoostClassifier         & 0.9361 $\pm$ 0.0126 & 0.5362 $\pm$ 0.1246 & 0.6510 $\pm$ 0.0719 & 0.9349 $\pm$ 0.0127 \\ \hline
		Lasso                      & 0.9523 $\pm$ 0.0414 & 0.5065 $\pm$ 0.4817 & 0.7401 $\pm$ 0.2303 & 0.9524 $\pm$ 0.0416 \\ \hline
		SGDClassifier              & 0.9258 $\pm$ 0.0169 & 0.3860 $\pm$ 0.2692 & 0.6098 $\pm$ 0.0894 & 0.9281 $\pm$ 0.0162 \\ \hline
	\end{tabular}
\end{table*}

==> table/imbalance_benchmark_datasets.tex <==
\iffalse
% 58 long columns
\begin{table}[h!]
\centering
\caption{Specification of imbalance classification benchmark datasets.}
\label{tab:imbalance_benchmark_datasets}
\begin{scriptsize}
	\begin{tabular}{l|cccc}
		\hline
		\hline
		Datasets                                                                    & \begin{tabular}[c]{@{}c@{}}Imbalance\\ Ratio\end{tabular} & \begin{tabular}[c]{@{}c@{}}Number of \\ Attributes\end{tabular} & \begin{tabular}[c]{@{}c@{}}Number of \\ TrainData\end{tabular} & \begin{tabular}[c]{@{}c@{}}Number of \\ TestData\end{tabular} \\ \hline
		abalone19                                                                   & 129.44                                                    & 8                                                               & 3339                                                           & 835                                                           \\
		abalone9-18                                                                 & 16.4                                                      & 8                                                               & 584                                                            & 147                                                           \\
		cleveland-0\_vs\_4                                                          & 12.62                                                     & 13                                                              & 177                                                            & 44                                                            \\
		ecoli-0-1-3-7\_vs\_2-6                                                      & 39.14                                                     & 7                                                               & 281                                                            & 70                                                            \\
		ecoli-0-1-4-6\_vs\_5                                                        & 13                                                        & 6                                                               & 224                                                            & 56                                                            \\
		ecoli-0-1-4-7\_vs\_2-3-5-6                                                  & 10.59                                                     & 7                                                               & 269                                                            & 67                                                            \\
		ecoli-0-1-4-7\_vs\_5-6                                                      & 12.28                                                     & 6                                                               & 266                                                            & 66                                                            \\
		ecoli-0-1\_vs\_2-3-5                                                        & 9.17                                                      & 7                                                               & 195                                                            & 49                                                            \\
		ecoli-0-1\_vs\_5                                                            & 11                                                        & 6                                                               & 192                                                            & 48                                                            \\
		ecoli-0-2-3-4\_vs\_5                                                        & 9.1                                                       & 7                                                               & 162                                                            & 40                                                            \\
		ecoli-0-2-6-7\_vs\_3-5                                                      & 9.18                                                      & 7                                                               & 179                                                            & 45                                                            \\
		ecoli-0-3-4-6\_vs\_5                                                        & 9.25                                                      & 7                                                               & 164                                                            & 41                                                            \\
		ecoli-0-3-4-7\_vs\_5-6                                                      & 9.28                                                      & 7                                                               & 206                                                            & 51                                                            \\
		ecoli-0-3-4\_vs\_5                                                          & 9                                                         & 7                                                               & 160                                                            & 40                                                            \\
		ecoli-0-4-6\_vs\_5                                                          & 9.15                                                      & 6                                                               & 162                                                            & 41                                                            \\
		ecoli-0-6-7\_vs\_3-5                                                        & 9.09                                                      & 7                                                               & 178                                                            & 44                                                            \\
		ecoli-0-6-7\_vs\_5                                                          & 10                                                        & 6                                                               & 176                                                            & 44                                                            \\
		ecoli3                                                                      & 8.6                                                       & 7                                                               & 269                                                            & 67                                                            \\
		glass-0-1-2-3\_vs\_4-5-6                                                    & 3.2                                                       & 9                                                               & 171                                                            & 43                                                            \\
		glass-0-1-4-6\_vs\_2                                                        & 11.06                                                     & 9                                                               & 164                                                            & 41                                                            \\
		glass-0-1-5\_vs\_2                                                          & 9.12                                                      & 9                                                               & 138                                                            & 34                                                            \\
		glass-0-1-6\_vs\_2                                                          & 10.29                                                     & 9                                                               & 154                                                            & 38                                                            \\
		glass-0-1-6\_vs\_5                                                          & 19.44                                                     & 9                                                               & 147                                                            & 37                                                            \\
		glass-0-4\_vs\_5                                                            & 9.22                                                      & 9                                                               & 74                                                             & 18                                                            \\
		glass-0-6\_vs\_5                                                            & 11                                                        & 9                                                               & 86                                                             & 22                                                            \\
		glass0                                                                      & 2.06                                                      & 9                                                               & 171                                                            & 43                                                            \\
		glass1                                                                      & 1.82                                                      & 9                                                               & 171                                                            & 43                                                            \\
		glass2                                                                      & 11.59                                                     & 9                                                               & 171                                                            & 43                                                            \\
		glass4                                                                      & 15.47                                                     & 9                                                               & 171                                                            & 43                                                            \\
		glass5                                                                      & 22.78                                                     & 9                                                               & 171                                                            & 43                                                            \\
		glass6                                                                      & 6.38                                                      & 9                                                               & 171                                                            & 43                                                            \\
		haberman                                                                    & 2.78                                                      & 3                                                               & 245                                                            & 61                                                            \\
		iris0                                                                       & 2                                                         & 4                                                               & 120                                                            & 30                                                            \\
		\begin{tabular}[c]{@{}c@{}}led7digit-0-2-4-5-6-7\\ -8-9\_vs\_1\end{tabular} & 10.97                                                     & 7                                                               & 354                                                            & 89                                                            \\
		new-thyroid1                                                                & 5.14                                                      & 5                                                               & 172                                                            & 43                                                            \\
		newthyroid2                                                                 & 5.14                                                      & 5                                                               & 172                                                            & 43                                                            \\
		page-blocks-1-3\_vs\_4                                                      & 15.86                                                     & 10                                                              & 378                                                            & 94                                                            \\
		page-blocks0                                                                & 8.79                                                      & 10                                                              & 4378                                                           & 1094                                                          \\
		pima                                                                        & 1.87                                                      & 8                                                               & 614                                                            & 154                                                           \\
		segment0                                                                    & 6.02                                                      & 19                                                              & 1846                                                           & 462                                                           \\
		shuttle-c0-vs-c4                                                            & 13.87                                                     & 9                                                               & 1463                                                           & 366                                                           \\
		shuttle-c2-vs-c4                                                            & 20.5                                                      & 9                                                               & 2653                                                           & 663                                                           \\
		vehicle0                                                                    & 3.25                                                      & 18                                                              & 677                                                            & 169                                                           \\
		vowel0                                                                      & 9.98                                                      & 13                                                              & 790                                                            & 198                                                           \\
		wisconsin                                                                   & 1.86                                                      & 9                                                               & 546                                                            & 137                                                           \\
		yeast-0-2-5-6\_vs\_3-7-8-9                                                  & 9.14                                                      & 8                                                               & 803                                                            & 201                                                           \\
		yeast-0-2-5-7-9\_vs\_3-6-8                                                  & 9.14                                                      & 8                                                               & 803                                                            & 201                                                           \\
		yeast-0-3-5-9\_vs\_7-8                                                      & 9.12                                                      & 8                                                               & 405                                                            & 101                                                           \\
		yeast-0-5-6-7-9\_vs\_4                                                      & 9.35                                                      & 8                                                               & 422                                                            & 106                                                           \\
		yeast-1-2-8-9\_vs\_7                                                        & 30.57                                                     & 8                                                               & 758                                                            & 189                                                           \\
		yeast-1-4-5-8\_vs\_7                                                        & 22.1                                                      & 8                                                               & 554                                                            & 139                                                           \\
		yeast-1\_vs\_7                                                              & 14.3                                                      & 7                                                               & 367                                                            & 92                                                            \\
		yeast-2\_vs\_4                                                              & 9.08                                                      & 8                                                               & 411                                                            & 103                                                           \\
		yeast-2\_vs\_8                                                              & 23.1                                                      & 8                                                               & 386                                                            & 96                                                            \\
		yeast1                                                                      & 2.46                                                      & 8                                                               & 1187                                                           & 297                                                           \\
		yeast3                                                                      & 8.1                                                       & 8                                                               & 1187                                                           & 297                                                           \\
		yeast4                                                                      & 28.1                                                      & 8                                                               & 1187                                                           & 297                                                           \\
		yeast5                                                                      & 32.73                                                     & 8                                                               & 1187                                                           & 297\\
		\hline                                                          
	\end{tabular}
\end{scriptsize}
\end{table}
\fi

% 29 two columns
\begin{table}[h!]
	\centering
\caption{Specification of imbalance classification benchmark datasets.}
\label{tab:imbalance_benchmark_datasets}
\begin{tiny}
	\begin{tabular}{l|cccc|l|cccc}
		\hline
		\hline
		\multicolumn{1}{c|}{Datasets} & \multicolumn{1}{c}{IR} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\# of\\ Attributes\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\# of\\ TrainData\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\# of\\ TestData\end{tabular}} & \multicolumn{1}{c|}{Datasets}                                                & \multicolumn{1}{c}{IR} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\# of\\ Attributes\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\# of\\ TrainData\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\#of\\ TestData\end{tabular}} \\ \hline
		abalone19                  & 129.44                                                    & 8                                                              & 3339                                                          & 835                                                          & glass5                                                                      & 22.78                                                     & 9                                                              & 171                                                           & 43                                                           \\
		abalone9-18                & 16.4                                                      & 8                                                              & 584                                                           & 147                                                          & glass6                                                                      & 6.38                                                      & 9                                                              & 171                                                           & 43                                                           \\
		cleveland-0\_vs\_4         & 12.62                                                     & 13                                                             & 177                                                           & 44                                                           & haberman                                                                    & 2.78                                                      & 3                                                              & 245                                                           & 61                                                           \\
		ecoli-0-1-3-7\_vs\_2-6     & 39.14                                                     & 7                                                              & 281                                                           & 70                                                           & iris0                                                                       & 2                                                         & 4                                                              & 120                                                           & 30                                                           \\
		ecoli-0-1-4-6\_vs\_5       & 13                                                        & 6                                                              & 224                                                           & 56                                                           & \begin{tabular}[c]{@{}l@{}}led7digit-0-2-4-5-6-7\\ -8-9\_vs\_1\end{tabular} & 10.97                                                     & 7                                                              & 354                                                           & 89                                                           \\
		ecoli-0-1-4-7\_vs\_2-3-5-6 & 10.59                                                     & 7                                                              & 269                                                           & 67                                                           & new-thyroid1                                                                & 5.14                                                      & 5                                                              & 172                                                           & 43                                                           \\
		ecoli-0-1-4-7\_vs\_5-6     & 12.28                                                     & 6                                                              & 266                                                           & 66                                                           & newthyroid2                                                                 & 5.14                                                      & 5                                                              & 172                                                           & 43                                                           \\
		ecoli-0-1\_vs\_2-3-5       & 9.17                                                      & 7                                                              & 195                                                           & 49                                                           & page-blocks-1-3\_vs\_4                                                      & 15.86                                                     & 10                                                             & 378                                                           & 94                                                           \\
		ecoli-0-1\_vs\_5           & 11                                                        & 6                                                              & 192                                                           & 48                                                           & page-blocks0                                                                & 8.79                                                      & 10                                                             & 4378                                                          & 1094                                                         \\
		ecoli-0-2-3-4\_vs\_5       & 9.1                                                       & 7                                                              & 162                                                           & 40                                                           & pima                                                                        & 1.87                                                      & 8                                                              & 614                                                           & 154                                                          \\
		ecoli-0-2-6-7\_vs\_3-5     & 9.18                                                      & 7                                                              & 179                                                           & 45                                                           & segment0                                                                    & 6.02                                                      & 19                                                             & 1846                                                          & 462                                                          \\
		ecoli-0-3-4-6\_vs\_5       & 9.25                                                      & 7                                                              & 164                                                           & 41                                                           & shuttle-c0-vs-c4                                                            & 13.87                                                     & 9                                                              & 1463                                                          & 366                                                          \\
		ecoli-0-3-4-7\_vs\_5-6     & 9.28                                                      & 7                                                              & 206                                                           & 51                                                           & shuttle-c2-vs-c4                                                            & 20.5                                                      & 9                                                              & 2653                                                          & 663                                                          \\
		ecoli-0-3-4\_vs\_5         & 9                                                         & 7                                                              & 160                                                           & 40                                                           & vehicle0                                                                    & 3.25                                                      & 18                                                             & 677                                                           & 169                                                          \\
		ecoli-0-4-6\_vs\_5         & 9.15                                                      & 6                                                              & 162                                                           & 41                                                           & vowel0                                                                      & 9.98                                                      & 13                                                             & 790                                                           & 198                                                          \\
		ecoli-0-6-7\_vs\_3-5       & 9.09                                                      & 7                                                              & 178                                                           & 44                                                           & wisconsin                                                                   & 1.86                                                      & 9                                                              & 546                                                           & 137                                                          \\
		ecoli-0-6-7\_vs\_5         & 10                                                        & 6                                                              & 176                                                           & 44                                                           & yeast-0-2-5-6\_vs\_3-7-8-9                                                  & 9.14                                                      & 8                                                              & 803                                                           & 201                                                          \\
		ecoli3                     & 8.6                                                       & 7                                                              & 269                                                           & 67                                                           & yeast-0-2-5-7-9\_vs\_3-6-8                                                  & 9.14                                                      & 8                                                              & 803                                                           & 201                                                          \\
		glass-0-1-2-3\_vs\_4-5-6   & 3.2                                                       & 9                                                              & 171                                                           & 43                                                           & yeast-0-3-5-9\_vs\_7-8                                                      & 9.12                                                      & 8                                                              & 405                                                           & 101                                                          \\
		glass-0-1-4-6\_vs\_2       & 11.06                                                     & 9                                                              & 164                                                           & 41                                                           & yeast-0-5-6-7-9\_vs\_4                                                      & 9.35                                                      & 8                                                              & 422                                                           & 106                                                          \\
		glass-0-1-5\_vs\_2         & 9.12                                                      & 9                                                              & 138                                                           & 34                                                           & yeast-1-2-8-9\_vs\_7                                                        & 30.57                                                     & 8                                                              & 758                                                           & 189                                                          \\
		glass-0-1-6\_vs\_2         & 10.29                                                     & 9                                                              & 154                                                           & 38                                                           & yeast-1-4-5-8\_vs\_7                                                        & 22.1                                                      & 8                                                              & 554                                                           & 139                                                          \\
		glass-0-1-6\_vs\_5         & 19.44                                                     & 9                                                              & 147                                                           & 37                                                           & yeast-1\_vs\_7                                                              & 14.3                                                      & 7                                                              & 367                                                           & 92                                                           \\
		glass-0-4\_vs\_5           & 9.22                                                      & 9                                                              & 74                                                            & 18                                                           & yeast-2\_vs\_4                                                              & 9.08                                                      & 8                                                              & 411                                                           & 103                                                          \\
		glass-0-6\_vs\_5           & 11                                                        & 9                                                              & 86                                                            & 22                                                           & yeast-2\_vs\_8                                                              & 23.1                                                      & 8                                                              & 386                                                           & 96                                                           \\
		glass0                     & 2.06                                                      & 9                                                              & 171                                                           & 43                                                           & yeast1                                                                      & 2.46                                                      & 8                                                              & 1187                                                          & 297                                                          \\
		glass1                     & 1.82                                                      & 9                                                              & 171                                                           & 43                                                           & yeast3                                                                      & 8.1                                                       & 8                                                              & 1187                                                          & 297                                                          \\
		glass2                     & 11.59                                                     & 9                                                              & 171                                                           & 43                                                           & yeast4                                                                      & 28.1                                                      & 8                                                              & 1187                                                          & 297                                                          \\
		glass4                     & 15.47                                                     & 9                                                              & 171                                                           & 43                                                           & yeast5                                                                      & 32.73                                                     & 8                                                              & 1187                                                          & 297\\
		\hline                                                         
	\end{tabular}
\end{tiny}
\end{table}

==> table/imbalance_benchmark_results_accuracy.tex <==
\iffalse
\begin{table*}[t]
\centering
\caption{Comparison of simulation results of ECSDBN and other methods on 58 KEEL benchmark datasets in terms of test accuracy.}
\begin{scriptsize}
\label{tab:imbalance_benchmark_result_accuracy}
	\begin{tabular}{l|ccccccc}
		\hline
		\hline
		Datasets      & \begin{tabular}[c]{@{}c@{}} ECSDBN\end{tabular} & DBN                    & ADASYN-DBN      & SMOTE-DBN     & \begin{tabular}[c]{@{}c@{}}SMOTE -borderline1\\-DBN \end{tabular} & \begin{tabular}[c]{@{}c@{}}SMOTE-borderline2\\-DBN \end{tabular} & \begin{tabular}[c]{@{}c@{}}SMOTE-SVM\\-DBN \end{tabular} \\ \hline
		%abalone19 & \textbf{0.9474 $\pm$ 0.3114} & 0.9185 $\pm$ 0.4152          & 0.9140 $\pm$ 0.0000 & 0.7152 $\pm$ 0.1070 & 0.8360 $\pm$ 0.1815 & 0.8016 $\pm$ 0.1105 & 0.8850 $\pm$ 0.0514 \\
		abalone9-18 & 0.9307 $\pm$ 0.0048 & \textbf{0.9403 $\pm$ 0.0045} & 0.7674 $\pm$ 0.0061$^\dag$ & 0.6510 $\pm$ 0.0457 & 0.7217 $\pm$ 0.0754$^\dag$ & 0.7014 $\pm$ 0.0954$^\dag$ & 0.7033 $\pm$ 0.0177$^\dag$ \\
		cleveland-0\_vs\_4 & \textbf{0.9858 $\pm$ 0.0115} & 0.9467 $\pm$ 0.0115 & 0.6939 $\pm$ 0.1419 & 0.7585 $\pm$ 0.2254 & 0.8317 $\pm$ 0.2145$^\dag$ & 0.7915 $\pm$ 0.2242$^\dag$ & 0.8293 $\pm$ 0.1898 \\
		ecoli-0-1-3-7\_vs\_2-6 & 0.9697 $\pm$ 0.0001 & \textbf{0.9859 $\pm$ 0.0052} & 0.9031 $\pm$ 0.1466$^\dag$ & 0.8482 $\pm$ 0.1837 & 0.8438 $\pm$ 0.1797$^\dag$ & 0.7810 $\pm$ 0.2407$^\dag$ & 0.9188 $\pm$ 0.0944 \\
		ecoli-0-1-4-6\_vs\_5 & 0.9582 $\pm$ 0.0001 & \textbf{0.9729 $\pm$ 0.0146} & 0.7273 $\pm$ 0.0000$^\dag$ & 0.8454 $\pm$ 0.1201$^\dag$ & 0.6092 $\pm$ 0.1756 & 0.7354 $\pm$ 0.1552$^\dag$ & 0.8500 $\pm$ 0.1328$^\dag$ \\
		ecoli-0-1-4-7\_vs\_2-3-5-6 & 0.9512 $\pm$ 0.0005 & \textbf{0.9647 $\pm$ 0.0000} & 0.6148 $\pm$ 0.0518 & 0.7260 $\pm$ 0.1890 & 0.8909 $\pm$ 0.1120 & 0.7253 $\pm$ 0.1524 & 0.7188 $\pm$ 0.2138 \\
		ecoli-0-1-4-7\_vs\_5-6 & \textbf{0.9622 $\pm$ 0.0002} & 0.9560 $\pm$ 0.0218          & 0.6661 $\pm$ 0.1150 & 0.7773 $\pm$ 0.1822 & 0.7929 $\pm$ 0.1830 & 0.8714 $\pm$ 0.0674 & 0.8019 $\pm$ 0.1890 \\
		ecoli-0-1\_vs\_2-3-5 & \textbf{0.9750 $\pm$ 0.0042} & 0.9689 $\pm$ 0.0000          & 0.7143 $\pm$ 0.0502 & 0.6491 $\pm$ 0.1826 & 0.7209 $\pm$ 0.1478 & 0.6209 $\pm$ 0.1444 & 0.6782 $\pm$ 0.2011 \\
		ecoli-0-1\_vs\_5 & 0.9498 $\pm$ 0.0049 & \textbf{0.9686 $\pm$ 0.0058} & 0.7200 $\pm$ 0.0000 & 0.8318 $\pm$ 0.1031 & 0.8091 $\pm$ 0.1695 & 0.7236 $\pm$ 0.1463 & 0.8900 $\pm$ 0.1542 \\
		ecoli-0-2-3-4\_vs\_5 & \textbf{0.9730 $\pm$ 0.0051} & 0.9029 $\pm$ 0.0101          & 0.6613 $\pm$ 0.0000 & 0.7253 $\pm$ 0.2016 & 0.5527 $\pm$ 0.1755 & 0.5560 $\pm$ 0.1098 & 0.7582 $\pm$ 0.1888 \\
		ecoli-0-2-6-7\_vs\_3-5 & 0.9475 $\pm$ 0.0067 & \textbf{0.9772 $\pm$ 0.0186} & 0.6049 $\pm$ 0.0000 & 0.5040 $\pm$ 0.1659 & 0.3851 $\pm$ 0.0189 & 0.3832 $\pm$ 0.0219 & 0.5505 $\pm$ 0.2114 \\
		ecoli-0-3-4-6\_vs\_5 & 0.9441 $\pm$ 0.0009 & \textbf{0.9596 $\pm$ 0.0284} & 0.6719 $\pm$ 0.0000 & 0.6860 $\pm$ 0.2410 & 0.6774 $\pm$ 0.1987 & 0.4785 $\pm$ 0.0913 & 0.6860 $\pm$ 0.2461 \\
		ecoli-0-3-4-7\_vs\_5-6 & 0.9358 $\pm$ 0.0079 & \textbf{0.9477 $\pm$ 0.0212} & 0.6158 $\pm$ 0.0832 & 0.6526 $\pm$ 0.1581 & 0.7155 $\pm$ 0.2012 & 0.6534 $\pm$ 0.1423 & 0.7250 $\pm$ 0.1821 \\
		ecoli-0-3-4\_vs\_5 & \textbf{0.9480 $\pm$ 0.0094} & 0.9007 $\pm$ 0.0079          & 0.6774 $\pm$ 0.0000 & 0.7344 $\pm$ 0.1932 & 0.7767 $\pm$ 0.1818 & 0.5689 $\pm$ 0.1526 & 0.8133 $\pm$ 0.2103 \\
		ecoli-0-4-6\_vs\_5 & \textbf{0.9741 $\pm$ 0.0293} & 0.9431 $\pm$ 0.0326          & 0.6984 $\pm$ 0.0000 & 0.6641 $\pm$ 0.1879 & 0.6391 $\pm$ 0.1857 & 0.5174 $\pm$ 0.1388 & 0.7391 $\pm$ 0.1852 \\
		ecoli-0-6-7\_vs\_3-5  & 0.9564 $\pm$ 0.0100 & \textbf{0.9696 $\pm$ 0.0121} & 0.6000 $\pm$ 0.0651 & 0.6300 $\pm$ 0.2025 & 0.5010 $\pm$ 0.1641 & 0.4720 $\pm$ 0.1193 & 0.7270 $\pm$ 0.1862 \\
		ecoli-0-6-7\_vs\_5 & 0.8664 $\pm$ 0.0077 & \textbf{0.9636 $\pm$ 0.0000} & 0.6184 $\pm$ 0.0000 & 0.5980 $\pm$ 0.1729 & 0.5470 $\pm$ 0.1443 & 0.4980 $\pm$ 0.1305 & 0.5730 $\pm$ 0.1939 \\
		ecoli3 & \textbf{0.9567 $\pm$ 0.0050} & 0.8936 $\pm$ 0.0082          & 0.5920 $\pm$ 0.0000 & 0.7212 $\pm$ 0.1748 & 0.7245 $\pm$ 0.1734 & 0.7033 $\pm$ 0.1344 & 0.8252 $\pm$ 0.1220 \\
		glass-0-1-2-3\_vs\_4-5-6 & 0.9597 $\pm$ 0.0074 & \textbf{0.9815 $\pm$ 0.0336} & 0.5795 $\pm$ 0.1187 & 0.7415 $\pm$ 0.1704 & 0.5402 $\pm$ 0.1153 & 0.4829 $\pm$ 0.0427 & 0.7768 $\pm$ 0.2115 \\
		glass-0-1-4-6\_vs\_2 & \textbf{0.9890 $\pm$ 0.0038} & 0.9038 $\pm$ 0.0000          & 0.7286 $\pm$ 0.0000 & 0.4915 $\pm$ 0.0580 & 0.4872 $\pm$ 0.0551 & 0.4777 $\pm$ 0.0498 & 0.6667 $\pm$ 0.0000 \\
		glass-0-1-5\_vs\_2 & \textbf{0.9356 $\pm$ 0.0214} & 0.8864 $\pm$ 0.0000          & 0.6066 $\pm$ 0.0000 & 0.5154 $\pm$ 0.0426 & 0.5128 $\pm$ 0.0472 & 0.4974 $\pm$ 0.0132 & 0.7193 $\pm$ 0.0000 \\
		glass-0-1-6\_vs\_2 & 0.6711 $\pm$ 0.0002 & \textbf{0.8980 $\pm$ 0.0000} & 0.6667 $\pm$ 0.0000 & 0.4795 $\pm$ 0.0407 & 0.5273 $\pm$ 0.0398 & 0.5170 $\pm$ 0.0497 & 0.6377 $\pm$ 0.0000 \\
		glass-0-1-6\_vs\_5 & 0.6761 $\pm$ 0.0110 & \textbf{0.9364 $\pm$ 0.0000} & 0.5325 $\pm$ 0.0551 & 0.6432 $\pm$ 0.2084 & 0.6261 $\pm$ 0.2060 & 0.7011 $\pm$ 0.1824 & 0.7627 $\pm$ 0.0000 \\
		glass-0-4\_vs\_5 & \textbf{0.9346 $\pm$ 0.0001} & 0.8763 $\pm$ 0.0067          & 0.6000 $\pm$ 0.0935 & 0.5524 $\pm$ 0.1713 & 0.5286 $\pm$ 0.1475 & 0.5000 $\pm$ 0.0502 & 0.5738 $\pm$ 0.2204 \\
		glass-0-6\_vs\_5 & \textbf{0.9636 $\pm$ 0.0488} & 0.8941 $\pm$ 0.0329          & 0.6409 $\pm$ 0.0144 & 0.5000 $\pm$ 0.0422 & 0.5760 $\pm$ 0.1632 & 0.5600 $\pm$ 0.1323 & 0.6180 $\pm$ 0.1153 \\
		glass0 & \textbf{0.9513 $\pm$ 0.0175} & 0.6664 $\pm$ 0.0250          & 0.5231 $\pm$ 0.0000 & 0.5542 $\pm$ 0.0963 & 0.5347 $\pm$ 0.0672 & 0.4681 $\pm$ 0.0262 & 0.5597 $\pm$ 0.0980 \\
		glass1 & \textbf{0.7196 $\pm$ 0.0282} & 0.6487 $\pm$ 0.0527          & 0.4444 $\pm$ 0.0000 & 0.5145 $\pm$ 0.0765 & 0.4986 $\pm$ 0.0730 & 0.5101 $\pm$ 0.0658 & 0.5246 $\pm$ 0.0482 \\
		glass2 & \textbf{0.9721 $\pm$ 0.0001} & 0.9091 $\pm$ 0.0000          & 0.6216 $\pm$ 0.0000 & 0.4485 $\pm$ 0.0630 & 0.4768 $\pm$ 0.0916 & 0.4424 $\pm$ 0.0506 & 0.7538 $\pm$ 0.0000 \\
		glass4 & \textbf{0.9717 $\pm$ 0.0088} & 0.9276 $\pm$ 0.0103          & 0.6024 $\pm$ 0.0151 & 0.6851 $\pm$ 0.2207 & 0.6733 $\pm$ 0.2186 & 0.6495 $\pm$ 0.2120 & 0.7667 $\pm$ 0.0205 \\
		glass5 & \textbf{0.9680 $\pm$ 0.0002} & 0.9455 $\pm$ 0.0088          & 0.6000 $\pm$ 0.0000 & 0.6058 $\pm$ 0.1948 & 0.6330 $\pm$ 0.1653 & 0.6495 $\pm$ 0.1836 & 0.7671 $\pm$ 0.0000 \\
		glass6 & \textbf{0.9732 $\pm$ 0.0002} & 0.8613 $\pm$ 0.0077          & 0.6821 $\pm$ 0.0622 & 0.7570 $\pm$ 0.1686 & 0.7118 $\pm$ 0.2084 & 0.7237 $\pm$ 0.1157 & 0.7656 $\pm$ 0.1745 \\
		haberman & \textbf{0.9821 $\pm$ 0.0001} & 0.7301 $\pm$ 0.0041          & 0.6162 $\pm$ 0.0000 & 0.4655 $\pm$ 0.0385 & 0.4478 $\pm$ 0.0140 & 0.5035 $\pm$ 0.0450 & 0.4841 $\pm$ 0.0336 \\
		iris0 & \textbf{0.9363 $\pm$ 0.0050} & 0.7227 $\pm$ 0.0000          & 0.6842 $\pm$ 0.0000 & 0.9340 $\pm$ 0.1708 & 0.7158 $\pm$ 0.0999 & 0.7447 $\pm$ 0.1278 & 0.6256 $\pm$ 0.1913 \\
		\begin{tabular}[c]{@{}l@{}}led7digit-0-2-4-5-6-7\\ -8-9\_vs\_1\end{tabular} & 0.7385 $\pm$ 0.0063 & \textbf{0.9141 $\pm$ 0.0075} & 0.8211 $\pm$ 0.0075 & 0.8722 $\pm$ 0.0070 & 0.8877 $\pm$ 0.1129 & 0.8291 $\pm$ 0.0925 & 0.9034 $\pm$ 0.0048 \\
		new-thyroid1 & \textbf{0.9681 $\pm$ 0.0026} & 0.8451 $\pm$ 0.0000          & 0.4815 $\pm$ 0.0000 & 0.6244 $\pm$ 0.1967 & 0.4867 $\pm$ 0.0729 & 0.4844 $\pm$ 0.0420 & 0.4911 $\pm$ 0.0491 \\
		newthyroid2 & \textbf{0.9870 $\pm$ 0.0153} & 0.8460 $\pm$ 0.0000          & 0.4815 $\pm$ 0.0000 & 0.5478 $\pm$ 0.1106 & 0.5011 $\pm$ 0.1051 & 0.4733 $\pm$ 0.0375 & 0.5100 $\pm$ 0.0686 \\
		page-blocks-1-3\_vs\_4 & \textbf{0.9796 $\pm$ 0.0089} & 0.9419 $\pm$ 0.0011          & 0.7617 $\pm$ 0.0673 & 0.6860 $\pm$ 0.1413 & 0.8414 $\pm$ 0.0687 & 0.7874 $\pm$ 0.1129 & 0.7450 $\pm$ 0.0213 \\
		page-blocks0 & 0.8639 $\pm$ 0.0028 & \textbf{0.9048 $\pm$ 0.0000} & 0.8312 $\pm$ 0.0129 & 0.8597 $\pm$ 0.0149 & 0.8059 $\pm$ 0.0151 & 0.6984 $\pm$ 0.1074 & 0.8499 $\pm$ 0.0292 \\
		pima & \textbf{0.9630 $\pm$ 0.0105} & 0.6555 $\pm$ 0.0192          & 0.5766 $\pm$ 0.0288 & 0.6188 $\pm$ 0.0637 & 0.5608 $\pm$ 0.0629 & 0.5232 $\pm$ 0.0651 & 0.5184 $\pm$ 0.0618 \\
		segment0 & \textbf{0.9546 $\pm$ 0.0054} & 0.8630 $\pm$ 0.0007          & 0.9197 $\pm$ 0.0167 & 0.8235 $\pm$ 0.2277 & 0.8776 $\pm$ 0.1310 & 0.8055 $\pm$ 0.1055 & 0.9385 $\pm$ 0.0132 \\
		shuttle-c0-vs-c4 & 0.9175 $\pm$ 0.0001 & \textbf{0.9342 $\pm$ 0.0000} & 0.9389 $\pm$ 0.0000 & 0.8971 $\pm$ 0.2170 & 0.9391 $\pm$ 0.0007 & 0.9393 $\pm$ 0.0009 & 0.8998 $\pm$ 0.1588 \\
		shuttle-c2-vs-c4 & \textbf{0.9701 $\pm$ 0.0050} & 0.9395 $\pm$ 0.0214          & 0.7180 $\pm$ 0.0569 & 0.6339 $\pm$ 0.1474 & 0.6032 $\pm$ 0.2077 & 0.6355 $\pm$ 0.1427 & 0.6875 $\pm$ 0.0000 \\
		vehicle0 & \textbf{0.8968 $\pm$ 0.0054} & 0.7740 $\pm$ 0.0066          & 0.7272 $\pm$ 0.0644 & 0.7577 $\pm$ 0.1420 & 0.7497 $\pm$ 0.1447 & 0.6735 $\pm$ 0.1276 & 0.7420 $\pm$ 0.1501 \\
		vowel0 & \textbf{0.9311 $\pm$ 0.0029} & 0.9089 $\pm$ 0.0114          & 0.8935 $\pm$ 0.0694 & 0.9053 $\pm$ 0.0207 & 0.8323 $\pm$ 0.1775 & 0.8472 $\pm$ 0.0184 & 0.8976 $\pm$ 0.0448 \\
		wisconsin & 0.9716 $\pm$ 0.0060 & 0.6910 $\pm$ 0.0054          & 0.9683 $\pm$ 0.0026 & 0.9216 $\pm$ 0.1482 & 0.9266 $\pm$ 0.1510 & 0.9203 $\pm$ 0.1477 & \textbf{0.9743 $\pm$ 0.0149} \\
		yeast-0-2-5-6\_vs\_3-7-8-9 & \textbf{0.9298 $\pm$ 0.0033} & 0.9019 $\pm$ 0.0028          & 0.6954 $\pm$ 0.0787 & 0.7576 $\pm$ 0.1378 & 0.7404 $\pm$ 0.0982 & 0.7775 $\pm$ 0.0075 & 0.8201 $\pm$ 0.0891 \\
		yeast-0-2-5-7-9\_vs\_3-6-8 & \textbf{0.9577 $\pm$ 0.0074} & 0.9047 $\pm$ 0.0073          & 0.7416 $\pm$ 0.1150 & 0.7945 $\pm$ 0.1842 & 0.6722 $\pm$ 0.1298 & 0.6667 $\pm$ 0.1163 & 0.8285 $\pm$ 0.1103 \\
		yeast-0-3-5-9\_vs\_7-8 & \textbf{0.9916 $\pm$ 0.0133} & 0.8976 $\pm$ 0.0041          & 0.6725 $\pm$ 0.0000 & 0.6136 $\pm$ 0.0577 & 0.5952 $\pm$ 0.1207 & 0.5649 $\pm$ 0.0980 & 0.6333 $\pm$ 0.0516 \\
		yeast-0-5-6-7-9\_vs\_4 & 0.7561 $\pm$ 0.0075 & \textbf{0.9030 $\pm$ 0.0055} & 0.6674 $\pm$ 0.0118 & 0.8121 $\pm$ 0.0260 & 0.8280 $\pm$ 0.0499 & 0.7285 $\pm$ 0.1245 & 0.8385 $\pm$ 0.1318 \\
		yeast-1-2-8-9\_vs\_7 & 0.9279 $\pm$ 0.0028 & \textbf{0.9664 $\pm$ 0.0103} & 0.7098 $\pm$ 0.0000 & 0.6614 $\pm$ 0.1196 & 0.6963 $\pm$ 0.0784 & 0.6229 $\pm$ 0.0987 & 0.7111 $\pm$ 0.0000 \\
		yeast-1-4-5-8\_vs\_7 & \textbf{0.9661 $\pm$ 0.0001} & 0.9540 $\pm$ 0.0082          & 0.7308 $\pm$ 0.0000 & 0.5422 $\pm$ 0.0833 & 0.6440 $\pm$ 0.0705 & 0.5542 $\pm$ 0.0676 & 0.7325 $\pm$ 0.0000 \\
		yeast-1\_vs\_7 & \textbf{0.9715 $\pm$ 0.0134} & 0.9371 $\pm$ 0.0013          & 0.6325 $\pm$ 0.0000 & 0.6884 $\pm$ 0.0385 & 0.7163 $\pm$ 0.0534 & 0.6670 $\pm$ 0.0699 & 0.7958 $\pm$ 0.1101 \\
		yeast-2\_vs\_4 & \textbf{0.9825 $\pm$ 0.0037} & 0.9026 $\pm$ 0.0000          & 0.6684 $\pm$ 0.0054 & 0.8681 $\pm$ 0.0299 & 0.6457 $\pm$ 0.1348 & 0.6159 $\pm$ 0.0910 & 0.8095 $\pm$ 0.1702 \\
		yeast-2\_vs\_8 & 0.9598 $\pm$ 0.0001 & \textbf{0.9917 $\pm$ 0.0033} & 0.8243 $\pm$ 0.0154 & 0.6883 $\pm$ 0.1186 & 0.5320 $\pm$ 0.0734 & 0.5255 $\pm$ 0.0911 & 0.6662 $\pm$ 0.0786 \\
		yeast1 & 0.7122 $\pm$ 0.0107 & \textbf{0.7125 $\pm$ 0.0000} & 0.5518 $\pm$ 0.0107 & 0.5278 $\pm$ 0.1033 & 0.5072 $\pm$ 0.0544 & 0.4867 $\pm$ 0.0474 & 0.6106 $\pm$ 0.0916 \\
		yeast3 & 0.8906 $\pm$ 0.0034 & \textbf{0.8911 $\pm$ 0.0042} & 0.6316 $\pm$ 0.0000 & 0.7808 $\pm$ 0.1711 & 0.6965 $\pm$ 0.1725 & 0.6321 $\pm$ 0.1174 & 0.6378 $\pm$ 0.1809 \\
		yeast4 & \textbf{0.9651 $\pm$ 0.0023} & 0.9651 $\pm$ 0.0028          & 0.8048 $\pm$ 0.1011 & 0.8230 $\pm$ 0.1177 & 0.8813 $\pm$ 0.1298 & 0.8996 $\pm$ 0.0027 & 0.9291 $\pm$ 0.0032 \\
		yeast5 & 0.9704 $\pm$ 0.0023 & \textbf{0.9728 $\pm$ 0.0020} & 0.9606 $\pm$ 0.0008 & 0.8715 $\pm$ 0.1976 & 0.8703 $\pm$ 0.1948 & 0.9272 $\pm$ 0.0013 & 0.9238 $\pm$ 0.1489\\
		\hline
		Average Ranking & \textbf{1.6466} & 1.8190 & 5.0690 & 4.8017  & 5.1034 & 5.8448 & 3.7155 \\ 
		%Wilcoxon Signed-Rank Test & - & \textbf{6.66191E-03} &\textbf{6.89366E-11}				 & \textbf{1.15216E-10} & \textbf{1.21228E-10}				  & \textbf{6.21751E-11}				   & \textbf{4.25901E-10}  \\ 
		Holm-Post hoc Test & - & \textbf{3.60922E-03} & \textbf{3.44739E-11}
		 & \textbf{5.76082E-11} & \textbf{6.06238E-11}		  & \textbf{3.10875E-11}		   & \textbf{2.12982E-10}  \\
		\hline      
	\end{tabular}
\end{scriptsize}
\end{table*}
\fi
\begin{table*}[!t]
\centering
\caption{Comparison of simulation results of ECSDBN and other methods on 58 KEEL benchmark datasets in terms of test accuracy.}
\begin{scriptsize}
\label{tab:imbalance_benchmark_result_accuracy}
	\begin{tabular}{l|ccccccc}
		\hline
		\hline
		Datasets      & \begin{tabular}[c]{@{}c@{}} ECSDBN\end{tabular} & DBN                    & ADASYN-DBN      & SMOTE-DBN     & \begin{tabular}[c]{@{}c@{}}SMOTE -borderline1\\-DBN \end{tabular} & \begin{tabular}[c]{@{}c@{}}SMOTE-borderline2\\-DBN \end{tabular} & \begin{tabular}[c]{@{}c@{}}SMOTE-SVM\\-DBN \end{tabular} \\ \hline
		%abalone19 & \textbf{0.9474 $\pm$ 0.3114} & 0.9185 $\pm$ 0.4152          & 0.9140 $\pm$ 0.0000 & 0.7152 $\pm$ 0.1070 & 0.8360 $\pm$ 0.1815 & 0.8016 $\pm$ 0.1105 & 0.8850 $\pm$ 0.0514 \\
		abalone9-18 & 0.9307 $\pm$ 0.0048 & \textbf{0.9403 $\pm$ 0.0045} & 0.7674 $\pm$ 0.0061 & 0.6510 $\pm$ 0.0457 & 0.7217 $\pm$ 0.0754 & 0.7014 $\pm$ 0.0954 & 0.7033 $\pm$ 0.0177 \\
		cleveland-0\_vs\_4 & \textbf{0.9858 $\pm$ 0.0115} & 0.9467 $\pm$ 0.0115 & 0.6939 $\pm$ 0.1419 & 0.7585 $\pm$ 0.2254 & 0.8317 $\pm$ 0.2145 & 0.7915 $\pm$ 0.2242 & 0.8293 $\pm$ 0.1898 \\
		ecoli-0-1-3-7\_vs\_2-6 & 0.9697 $\pm$ 0.0001 & \textbf{0.9859 $\pm$ 0.0052} & 0.9031 $\pm$ 0.1466 & 0.8482 $\pm$ 0.1837 & 0.8438 $\pm$ 0.1797 & 0.7810 $\pm$ 0.2407 & 0.9188 $\pm$ 0.0944 \\
		ecoli-0-1-4-6\_vs\_5 & 0.9582 $\pm$ 0.0001 & \textbf{0.9729 $\pm$ 0.0146} & 0.7273 $\pm$ 0.0000 & 0.8454 $\pm$ 0.1201 & 0.6092 $\pm$ 0.1756 & 0.7354 $\pm$ 0.1552 & 0.8500 $\pm$ 0.1328 \\
		ecoli-0-1-4-7\_vs\_2-3-5-6 & 0.9512 $\pm$ 0.0005 & \textbf{0.9647 $\pm$ 0.0000} & 0.6148 $\pm$ 0.0518 & 0.7260 $\pm$ 0.1890 & 0.8909 $\pm$ 0.1120 & 0.7253 $\pm$ 0.1524 & 0.7188 $\pm$ 0.2138 \\
		ecoli-0-1-4-7\_vs\_5-6 & \textbf{0.9622 $\pm$ 0.0002} & 0.9560 $\pm$ 0.0218          & 0.6661 $\pm$ 0.1150 & 0.7773 $\pm$ 0.1822 & 0.7929 $\pm$ 0.1830 & 0.8714 $\pm$ 0.0674 & 0.8019 $\pm$ 0.1890 \\
		ecoli-0-1\_vs\_2-3-5 & \textbf{0.9750 $\pm$ 0.0042} & 0.9689 $\pm$ 0.0000          & 0.7143 $\pm$ 0.0502 & 0.6491 $\pm$ 0.1826 & 0.7209 $\pm$ 0.1478 & 0.6209 $\pm$ 0.1444 & 0.6782 $\pm$ 0.2011 \\
		ecoli-0-1\_vs\_5 & 0.9498 $\pm$ 0.0049 & \textbf{0.9686 $\pm$ 0.0058} & 0.7200 $\pm$ 0.0000 & 0.8318 $\pm$ 0.1031 & 0.8091 $\pm$ 0.1695 & 0.7236 $\pm$ 0.1463 & 0.8900 $\pm$ 0.1542 \\
		ecoli-0-2-3-4\_vs\_5 & \textbf{0.9730 $\pm$ 0.0051}$^\dag$ & 0.9029 $\pm$ 0.0101          & 0.6613 $\pm$ 0.0000 & 0.7253 $\pm$ 0.2016 & 0.5527 $\pm$ 0.1755 & 0.5560 $\pm$ 0.1098 & 0.7582 $\pm$ 0.1888 \\
		ecoli-0-2-6-7\_vs\_3-5 & 0.9475 $\pm$ 0.0067 & \textbf{0.9772 $\pm$ 0.0186} & 0.6049 $\pm$ 0.0000 & 0.5040 $\pm$ 0.1659 & 0.3851 $\pm$ 0.0189 & 0.3832 $\pm$ 0.0219 & 0.5505 $\pm$ 0.2114 \\
		ecoli-0-3-4-6\_vs\_5 & 0.9441 $\pm$ 0.0009 & \textbf{0.9596 $\pm$ 0.0284} & 0.6719 $\pm$ 0.0000 & 0.6860 $\pm$ 0.2410 & 0.6774 $\pm$ 0.1987 & 0.4785 $\pm$ 0.0913 & 0.6860 $\pm$ 0.2461 \\
		ecoli-0-3-4-7\_vs\_5-6 & 0.9358 $\pm$ 0.0079 & \textbf{0.9477 $\pm$ 0.0212} & 0.6158 $\pm$ 0.0832 & 0.6526 $\pm$ 0.1581 & 0.7155 $\pm$ 0.2012 & 0.6534 $\pm$ 0.1423 & 0.7250 $\pm$ 0.1821 \\
		ecoli-0-3-4\_vs\_5 & \textbf{0.9480 $\pm$ 0.0094} & 0.9007 $\pm$ 0.0079          & 0.6774 $\pm$ 0.0000 & 0.7344 $\pm$ 0.1932 & 0.7767 $\pm$ 0.1818 & 0.5689 $\pm$ 0.1526 & 0.8133 $\pm$ 0.2103 \\
		ecoli-0-4-6\_vs\_5 & \textbf{0.9741 $\pm$ 0.0293}$^\dag$ & 0.9431 $\pm$ 0.0326          & 0.6984 $\pm$ 0.0000 & 0.6641 $\pm$ 0.1879 & 0.6391 $\pm$ 0.1857 & 0.5174 $\pm$ 0.1388 & 0.7391 $\pm$ 0.1852 \\
		ecoli-0-6-7\_vs\_3-5  & 0.9564 $\pm$ 0.0100 & \textbf{0.9696 $\pm$ 0.0121} & 0.6000 $\pm$ 0.0651 & 0.6300 $\pm$ 0.2025 & 0.5010 $\pm$ 0.1641 & 0.4720 $\pm$ 0.1193 & 0.7270 $\pm$ 0.1862 \\
		ecoli-0-6-7\_vs\_5 & 0.8664 $\pm$ 0.0077 & \textbf{0.9636 $\pm$ 0.0000} & 0.6184 $\pm$ 0.0000 & 0.5980 $\pm$ 0.1729 & 0.5470 $\pm$ 0.1443 & 0.4980 $\pm$ 0.1305 & 0.5730 $\pm$ 0.1939 \\
		ecoli3 & \textbf{0.9567 $\pm$ 0.0050}$^\dag$ & 0.8936 $\pm$ 0.0082          & 0.5920 $\pm$ 0.0000 & 0.7212 $\pm$ 0.1748 & 0.7245 $\pm$ 0.1734 & 0.7033 $\pm$ 0.1344 & 0.8252 $\pm$ 0.1220 \\
		glass-0-1-2-3\_vs\_4-5-6 & 0.9597 $\pm$ 0.0074 & \textbf{0.9815 $\pm$ 0.0336} & 0.5795 $\pm$ 0.1187 & 0.7415 $\pm$ 0.1704 & 0.5402 $\pm$ 0.1153 & 0.4829 $\pm$ 0.0427 & 0.7768 $\pm$ 0.2115 \\
		glass-0-1-4-6\_vs\_2 & \textbf{0.9890 $\pm$ 0.0038}$^\dag$ & 0.9038 $\pm$ 0.0000          & 0.7286 $\pm$ 0.0000 & 0.4915 $\pm$ 0.0580 & 0.4872 $\pm$ 0.0551 & 0.4777 $\pm$ 0.0498 & 0.6667 $\pm$ 0.0000 \\
		glass-0-1-5\_vs\_2 & \textbf{0.9356 $\pm$ 0.0214}$^\dag$ & 0.8864 $\pm$ 0.0000          & 0.6066 $\pm$ 0.0000 & 0.5154 $\pm$ 0.0426 & 0.5128 $\pm$ 0.0472 & 0.4974 $\pm$ 0.0132 & 0.7193 $\pm$ 0.0000 \\
		glass-0-1-6\_vs\_2 & 0.6711 $\pm$ 0.0002 & \textbf{0.8980 $\pm$ 0.0000} & 0.6667 $\pm$ 0.0000 & 0.4795 $\pm$ 0.0407 & 0.5273 $\pm$ 0.0398 & 0.5170 $\pm$ 0.0497 & 0.6377 $\pm$ 0.0000 \\
		glass-0-1-6\_vs\_5 & 0.6761 $\pm$ 0.0110 & \textbf{0.9364 $\pm$ 0.0000} & 0.5325 $\pm$ 0.0551 & 0.6432 $\pm$ 0.2084 & 0.6261 $\pm$ 0.2060 & 0.7011 $\pm$ 0.1824 & 0.7627 $\pm$ 0.0000 \\
		glass-0-4\_vs\_5 & \textbf{0.9346 $\pm$ 0.0001}$^\dag$ & 0.8763 $\pm$ 0.0067          & 0.6000 $\pm$ 0.0935 & 0.5524 $\pm$ 0.1713 & 0.5286 $\pm$ 0.1475 & 0.5000 $\pm$ 0.0502 & 0.5738 $\pm$ 0.2204 \\
		glass-0-6\_vs\_5 & \textbf{0.9636 $\pm$ 0.0488}$^\dag$ & 0.8941 $\pm$ 0.0329          & 0.6409 $\pm$ 0.0144 & 0.5000 $\pm$ 0.0422 & 0.5760 $\pm$ 0.1632 & 0.5600 $\pm$ 0.1323 & 0.6180 $\pm$ 0.1153 \\
		glass0 & \textbf{0.9513 $\pm$ 0.0175}$^\dag$ & 0.6664 $\pm$ 0.0250          & 0.5231 $\pm$ 0.0000 & 0.5542 $\pm$ 0.0963 & 0.5347 $\pm$ 0.0672 & 0.4681 $\pm$ 0.0262 & 0.5597 $\pm$ 0.0980 \\
		glass1 & \textbf{0.7196 $\pm$ 0.0282}$^\dag$ & 0.6487 $\pm$ 0.0527          & 0.4444 $\pm$ 0.0000 & 0.5145 $\pm$ 0.0765 & 0.4986 $\pm$ 0.0730 & 0.5101 $\pm$ 0.0658 & 0.5246 $\pm$ 0.0482 \\
		glass2 & \textbf{0.9721 $\pm$ 0.0001}$^\dag$ & 0.9091 $\pm$ 0.0000          & 0.6216 $\pm$ 0.0000 & 0.4485 $\pm$ 0.0630 & 0.4768 $\pm$ 0.0916 & 0.4424 $\pm$ 0.0506 & 0.7538 $\pm$ 0.0000 \\
		glass4 & \textbf{0.9717 $\pm$ 0.0088}$^\dag$ & 0.9276 $\pm$ 0.0103          & 0.6024 $\pm$ 0.0151 & 0.6851 $\pm$ 0.2207 & 0.6733 $\pm$ 0.2186 & 0.6495 $\pm$ 0.2120 & 0.7667 $\pm$ 0.0205 \\
		glass5 & \textbf{0.9680 $\pm$ 0.0002} & 0.9455 $\pm$ 0.0088          & 0.6000 $\pm$ 0.0000 & 0.6058 $\pm$ 0.1948 & 0.6330 $\pm$ 0.1653 & 0.6495 $\pm$ 0.1836 & 0.7671 $\pm$ 0.0000 \\
		glass6 & \textbf{0.9732 $\pm$ 0.0002}$^\dag$ & 0.8613 $\pm$ 0.0077          & 0.6821 $\pm$ 0.0622 & 0.7570 $\pm$ 0.1686 & 0.7118 $\pm$ 0.2084 & 0.7237 $\pm$ 0.1157 & 0.7656 $\pm$ 0.1745 \\
		haberman & \textbf{0.9821 $\pm$ 0.0001}$^\dag$ & 0.7301 $\pm$ 0.0041          & 0.6162 $\pm$ 0.0000 & 0.4655 $\pm$ 0.0385 & 0.4478 $\pm$ 0.0140 & 0.5035 $\pm$ 0.0450 & 0.4841 $\pm$ 0.0336 \\
		iris0 & \textbf{0.9363 $\pm$ 0.0050} & 0.7227 $\pm$ 0.0000          & 0.6842 $\pm$ 0.0000 & 0.9340 $\pm$ 0.1708 & 0.7158 $\pm$ 0.0999 & 0.7447 $\pm$ 0.1278 & 0.6256 $\pm$ 0.1913 \\
		\begin{tabular}[c]{@{}l@{}}led7digit-0-2-4-5-6-7\\ -8-9\_vs\_1\end{tabular} & 0.7385 $\pm$ 0.0063 & \textbf{0.9141 $\pm$ 0.0075} & 0.8211 $\pm$ 0.0075 & 0.8722 $\pm$ 0.0070 & 0.8877 $\pm$ 0.1129 & 0.8291 $\pm$ 0.0925 & 0.9034 $\pm$ 0.0048 \\
		new-thyroid1 & \textbf{0.9681 $\pm$ 0.0026}$^\dag$ & 0.8451 $\pm$ 0.0000          & 0.4815 $\pm$ 0.0000 & 0.6244 $\pm$ 0.1967 & 0.4867 $\pm$ 0.0729 & 0.4844 $\pm$ 0.0420 & 0.4911 $\pm$ 0.0491 \\
		newthyroid2 & \textbf{0.9870 $\pm$ 0.0153}$^\dag$ & 0.8460 $\pm$ 0.0000          & 0.4815 $\pm$ 0.0000 & 0.5478 $\pm$ 0.1106 & 0.5011 $\pm$ 0.1051 & 0.4733 $\pm$ 0.0375 & 0.5100 $\pm$ 0.0686 \\
		page-blocks-1-3\_vs\_4 & \textbf{0.9796 $\pm$ 0.0089}$^\dag$ & 0.9419 $\pm$ 0.0011          & 0.7617 $\pm$ 0.0673 & 0.6860 $\pm$ 0.1413 & 0.8414 $\pm$ 0.0687 & 0.7874 $\pm$ 0.1129 & 0.7450 $\pm$ 0.0213 \\
		page-blocks0 & 0.8639 $\pm$ 0.0028 & \textbf{0.9048 $\pm$ 0.0000} & 0.8312 $\pm$ 0.0129 & 0.8597 $\pm$ 0.0149 & 0.8059 $\pm$ 0.0151 & 0.6984 $\pm$ 0.1074 & 0.8499 $\pm$ 0.0292 \\
		pima & \textbf{0.9630 $\pm$ 0.0105}$^\dag$ & 0.6555 $\pm$ 0.0192          & 0.5766 $\pm$ 0.0288 & 0.6188 $\pm$ 0.0637 & 0.5608 $\pm$ 0.0629 & 0.5232 $\pm$ 0.0651 & 0.5184 $\pm$ 0.0618 \\
		segment0 & \textbf{0.9546 $\pm$ 0.0054} & 0.8630 $\pm$ 0.0007          & 0.9197 $\pm$ 0.0167 & 0.8235 $\pm$ 0.2277 & 0.8776 $\pm$ 0.1310 & 0.8055 $\pm$ 0.1055 & 0.9385 $\pm$ 0.0132 \\
		shuttle-c0-vs-c4 & 0.9175 $\pm$ 0.0001 & \textbf{0.9342 $\pm$ 0.0000} & 0.9389 $\pm$ 0.0000 & 0.8971 $\pm$ 0.2170 & 0.9391 $\pm$ 0.0007 & 0.9393 $\pm$ 0.0009 & 0.8998 $\pm$ 0.1588 \\
		shuttle-c2-vs-c4 & \textbf{0.9701 $\pm$ 0.0050} & 0.9395 $\pm$ 0.0214          & 0.7180 $\pm$ 0.0569 & 0.6339 $\pm$ 0.1474 & 0.6032 $\pm$ 0.2077 & 0.6355 $\pm$ 0.1427 & 0.6875 $\pm$ 0.0000 \\
		vehicle0 & \textbf{0.8968 $\pm$ 0.0054}$^\dag$ & 0.7740 $\pm$ 0.0066          & 0.7272 $\pm$ 0.0644 & 0.7577 $\pm$ 0.1420 & 0.7497 $\pm$ 0.1447 & 0.6735 $\pm$ 0.1276 & 0.7420 $\pm$ 0.1501 \\
		vowel0 & \textbf{0.9311 $\pm$ 0.0029} & 0.9089 $\pm$ 0.0114          & 0.8935 $\pm$ 0.0694 & 0.9053 $\pm$ 0.0207 & 0.8323 $\pm$ 0.1775 & 0.8472 $\pm$ 0.0184 & 0.8976 $\pm$ 0.0448 \\
		wisconsin & 0.9716 $\pm$ 0.0060 & 0.6910 $\pm$ 0.0054          & 0.9683 $\pm$ 0.0026 & 0.9216 $\pm$ 0.1482 & 0.9266 $\pm$ 0.1510 & 0.9203 $\pm$ 0.1477 & \textbf{0.9743 $\pm$ 0.0149} \\
		yeast-0-2-5-6\_vs\_3-7-8-9 & \textbf{0.9298 $\pm$ 0.0033} & 0.9019 $\pm$ 0.0028          & 0.6954 $\pm$ 0.0787 & 0.7576 $\pm$ 0.1378 & 0.7404 $\pm$ 0.0982 & 0.7775 $\pm$ 0.0075 & 0.8201 $\pm$ 0.0891 \\
		yeast-0-2-5-7-9\_vs\_3-6-8 & \textbf{0.9577 $\pm$ 0.0074} & 0.9047 $\pm$ 0.0073          & 0.7416 $\pm$ 0.1150 & 0.7945 $\pm$ 0.1842 & 0.6722 $\pm$ 0.1298 & 0.6667 $\pm$ 0.1163 & 0.8285 $\pm$ 0.1103 \\
		yeast-0-3-5-9\_vs\_7-8 & \textbf{0.9916 $\pm$ 0.0133}$^\dag$ & 0.8976 $\pm$ 0.0041          & 0.6725 $\pm$ 0.0000 & 0.6136 $\pm$ 0.0577 & 0.5952 $\pm$ 0.1207 & 0.5649 $\pm$ 0.0980 & 0.6333 $\pm$ 0.0516 \\
		yeast-0-5-6-7-9\_vs\_4 & 0.7561 $\pm$ 0.0075 & \textbf{0.9030 $\pm$ 0.0055} & 0.6674 $\pm$ 0.0118 & 0.8121 $\pm$ 0.0260 & 0.8280 $\pm$ 0.0499 & 0.7285 $\pm$ 0.1245 & 0.8385 $\pm$ 0.1318 \\
		yeast-1-2-8-9\_vs\_7 & 0.9279 $\pm$ 0.0028 & \textbf{0.9664 $\pm$ 0.0103} & 0.7098 $\pm$ 0.0000 & 0.6614 $\pm$ 0.1196 & 0.6963 $\pm$ 0.0784 & 0.6229 $\pm$ 0.0987 & 0.7111 $\pm$ 0.0000 \\
		yeast-1-4-5-8\_vs\_7 & \textbf{0.9661 $\pm$ 0.0001} & 0.9540 $\pm$ 0.0082          & 0.7308 $\pm$ 0.0000 & 0.5422 $\pm$ 0.0833 & 0.6440 $\pm$ 0.0705 & 0.5542 $\pm$ 0.0676 & 0.7325 $\pm$ 0.0000 \\
		yeast-1\_vs\_7 & \textbf{0.9715 $\pm$ 0.0134}$^\dag$ & 0.9371 $\pm$ 0.0013          & 0.6325 $\pm$ 0.0000 & 0.6884 $\pm$ 0.0385 & 0.7163 $\pm$ 0.0534 & 0.6670 $\pm$ 0.0699 & 0.7958 $\pm$ 0.1101 \\
		yeast-2\_vs\_4 & \textbf{0.9825 $\pm$ 0.0037}$^\dag$ & 0.9026 $\pm$ 0.0000          & 0.6684 $\pm$ 0.0054 & 0.8681 $\pm$ 0.0299 & 0.6457 $\pm$ 0.1348 & 0.6159 $\pm$ 0.0910 & 0.8095 $\pm$ 0.1702 \\
		yeast-2\_vs\_8 & 0.9598 $\pm$ 0.0001 & \textbf{0.9917 $\pm$ 0.0033} & 0.8243 $\pm$ 0.0154 & 0.6883 $\pm$ 0.1186 & 0.5320 $\pm$ 0.0734 & 0.5255 $\pm$ 0.0911 & 0.6662 $\pm$ 0.0786 \\
		yeast1 & 0.7122 $\pm$ 0.0107 & \textbf{0.7125 $\pm$ 0.0000} & 0.5518 $\pm$ 0.0107 & 0.5278 $\pm$ 0.1033 & 0.5072 $\pm$ 0.0544 & 0.4867 $\pm$ 0.0474 & 0.6106 $\pm$ 0.0916 \\
		yeast3 & 0.8906 $\pm$ 0.0034 & \textbf{0.8911 $\pm$ 0.0042} & 0.6316 $\pm$ 0.0000 & 0.7808 $\pm$ 0.1711 & 0.6965 $\pm$ 0.1725 & 0.6321 $\pm$ 0.1174 & 0.6378 $\pm$ 0.1809 \\
		yeast4 & \textbf{0.9651 $\pm$ 0.0023} & 0.9651 $\pm$ 0.0028          & 0.8048 $\pm$ 0.1011 & 0.8230 $\pm$ 0.1177 & 0.8813 $\pm$ 0.1298 & 0.8996 $\pm$ 0.0027 & 0.9291 $\pm$ 0.0032 \\
		yeast5 & 0.9704 $\pm$ 0.0023 & \textbf{0.9728 $\pm$ 0.0020} & 0.9606 $\pm$ 0.0008 & 0.8715 $\pm$ 0.1976 & 0.8703 $\pm$ 0.1948 & 0.9272 $\pm$ 0.0013 & 0.9238 $\pm$ 0.1489\\
		\hline
		Average Rank & \textbf{1.6466} & 1.8190 & 5.0690 & 4.8017  & 5.1034 & 5.8448 & 3.7155 \\ 
		Win-lose-draw& - & 34-4-20 & 50-0-8 & 48-0-10 & 48-1-9 &	54-0-4    & 44-0-14    \\
		%Wilcoxon Signed-Rank Test & - & \textbf{6.66191E-03} &\textbf{6.89366E-11}				 & \textbf{1.15216E-10} & \textbf{1.21228E-10}				  & \textbf{6.21751E-11}				   & \textbf{4.25901E-10}  \\ 
		Holm post-hoc Test & - & \textbf{3.60922E-03} & \textbf{3.44739E-11}
		 & \textbf{5.76082E-11} & \textbf{6.06238E-11}		  & \textbf{3.10875E-11}		   & \textbf{2.12982E-10}  \\
		\hline      
	\end{tabular}
	\\
	$\dag$ indicates that the difference between the proposed algorithm and all other compared algorithm is statistically significant using pair-wised Wilcoxon rank sum test at the $5\%$ significance level.
\end{scriptsize}
\end{table*}


==> table/imbalance_benchmark_results_gmean.tex <==
\begin{table*}[!t]
\centering
\caption{Comparison of simulation results of ECSDBN and other methods on 58 KEEL benchmark datasets in terms of test G-mean.}
\label{tab:imbalance_benchmark_result_gmean}
\begin{scriptsize}
\begin{tabular}{l|ccccccc}
	\hline
	\hline
	Datasets                         & \begin{tabular}[c]{@{}c@{}}ECSDBN\end{tabular} & DBN           & ADASYN-DBN               & SMOTE-DBN              & \begin{tabular}[c]{@{}c@{}}SMOTE-borderline1\\ -DBN\end{tabular} & \begin{tabular}[c]{@{}c@{}}SMOTE-borderline2\\ -DBN\end{tabular} & \begin{tabular}[c]{@{}c@{}}SMOTE-SVM\\ -DBN\end{tabular} \\ \hline
	%abalone19                        & 0.0000 $\pm$ 0.0000                                             & 0.0000 $\pm$ 0.0000 & 0.0000 $\pm$ 0.0000          & 0.6537 $\pm$ 0.2419          & 0.7351 $\pm$ 0.3875                                                    & 0.7406 $\pm$ 0.2620                                                    & \textbf{0.7437 $\pm$ 0.2665}                                          \\
	abalone9-18                      & \textbf{0.7236 $\pm$ 0.0064}                                    & 0.0066 $\pm$ 0.0066 & 0.1422 $\pm$ 0.1565          & 0.6387 $\pm$ 0.0508          & 0.6638 $\pm$ 0.2352                                                    & 0.6266 $\pm$ 0.2518                                                    & 0.5989 $\pm$ 0.0441                                                   \\
	cleveland-0\_vs\_4               & \textbf{0.8596 $\pm$ 0.0180}                                    & 0.0222 $\pm$ 0.0222 & 0.2681 $\pm$ 0.4321          & 0.6411 $\pm$ 0.3960          & 0.7689 $\pm$ 0.3476                                                    & 0.6946 $\pm$ 0.4008                                                    & 0.6620 $\pm$ 0.4585                                                   \\
	ecoli-0-1-3-7\_vs\_2-6           & \textbf{0.9927 $\pm$ 0.0140}                                   & 0.0149 $\pm$ 0.0149 & 0.6970 $\pm$ 0.4810          & 0.7474 $\pm$ 0.3940          & 0.7419 $\pm$ 0.3913                                                    & 0.5795 $\pm$ 0.4997                                                    & 0.6626 $\pm$ 0.4573                                                   \\
	ecoli-0-1-4-6\_vs\_5             & \textbf{0.8944 $\pm$ 0.0113}                                   & 0.0084 $\pm$ 0.0084 & 0.0000 $\pm$ 0.0000          & 0.7910 $\pm$ 0.2817          & 0.3182 $\pm$ 0.4014                                                    & 0.6245 $\pm$ 0.3428                                                    & 0.8010 $\pm$ 0.2823                                                   \\
	ecoli-0-1-4-7\_vs\_2-3-5-6       & \textbf{0.8604 $\pm$ 0.0176}                                    & 0.0189 $\pm$ 0.0189 & 0.0639 $\pm$ 0.2020          & 0.6336 $\pm$ 0.3174          & 0.8902 $\pm$ 0.1221                                                    & 0.6303 $\pm$ 0.3097                                                    & 0.5635 $\pm$ 0.4223                                                   \\
	ecoli-0-1-4-7\_vs\_5-6           & \textbf{0.9076 $\pm$ 0.0157}                                    & 0.0183 $\pm$ 0.0183 & 0.2073 $\pm$ 0.3545          & 0.6931 $\pm$ 0.3285          & 0.6988 $\pm$ 0.3432                                                    & 0.8686 $\pm$ 0.0800                                                    & 0.7035 $\pm$ 0.3792                                                   \\
	ecoli-0-1\_vs\_2-3-5             & \textbf{0.9129 $\pm$ 0.0177}$^\dag$                                    & 0.0169 $\pm$ 0.0169 & 0.1240 $\pm$ 0.2615          & 0.3940 $\pm$ 0.4252          & 0.5898 $\pm$ 0.3323                                                    & 0.4235 $\pm$ 0.3268                                                    & 0.4553 $\pm$ 0.4246                                                   \\
	ecoli-0-1\_vs\_5                 & \textbf{0.8516 $\pm$ 0.0153}                                    & 0.0145 $\pm$ 0.0145 & 0.0000 $\pm$ 0.0000          & 0.8232 $\pm$ 0.1246          & 0.7070 $\pm$ 0.3753                                                    & 0.6193 $\pm$ 0.2982                                                    & 0.8439 $\pm$ 0.2987                                                   \\
	ecoli-0-2-3-4\_vs\_5             & \textbf{0.8374 $\pm$ 0.0126}                                    & 0.0159 $\pm$ 0.0159 & 0.0000 $\pm$ 0.0000          & 0.5807 $\pm$ 0.4091          & 0.2328 $\pm$ 0.3821                                                    & 0.3059 $\pm$ 0.3169                                                    & 0.6557 $\pm$ 0.3635                                                   \\
	ecoli-0-2-6-7\_vs\_3-5           & \textbf{0.9192 $\pm$ 0.0170}$^\dag$                                    & 0.0186 $\pm$ 0.0186 & 0.0000 $\pm$ 0.0000          & 0.3060 $\pm$ 0.3511          & 0.0534 $\pm$ 0.1127                                                    & 0.0333 $\pm$ 0.1054                                                    & 0.3763 $\pm$ 0.4055                                                   \\
	ecoli-0-3-4-6\_vs\_5             & \textbf{0.9324 $\pm$ 0.0146}$^\dag$                                    & 0.0156 $\pm$ 0.0156 & 0.0000 $\pm$ 0.0000          & 0.5209 $\pm$ 0.4542          & 0.5688 $\pm$ 0.3637                                                    & 0.2062 $\pm$ 0.2568                                                    & 0.5159 $\pm$ 0.4543                                                   \\
	ecoli-0-3-4-7\_vs\_5-6           & \textbf{0.9065 $\pm$ 0.0117}$^\dag$                                    & 0.0138 $\pm$ 0.0138 & 0.0801 $\pm$ 0.2532          & 0.4437 $\pm$ 0.3603          & 0.5069 $\pm$ 0.4458                                                    & 0.4702 $\pm$ 0.3572                                                    & 0.5618 $\pm$ 0.4039                                                   \\
	ecoli-0-3-4\_vs\_5               & \textbf{0.9133 $\pm$ 0.0134}                                    & 0.9098 $\pm$ 0.0578 & 0.0000 $\pm$ 0.0000          & 0.6126 $\pm$ 0.3645          & 0.6592 $\pm$ 0.3724                                                    & 0.2383 $\pm$ 0.3595                                                    & 0.7176 $\pm$ 0.3933                                                   \\
	ecoli-0-4-6\_vs\_5               & \textbf{0.9746 $\pm$ 0.0157}$^\dag$                                    & 0.0156 $\pm$ 0.0156 & 0.0000 $\pm$ 0.0000          & 0.4899 $\pm$ 0.3660          & 0.4509 $\pm$ 0.3661                                                    & 0.2919 $\pm$ 0.3219                                                    & 0.6553 $\pm$ 0.3237                                                   \\
	ecoli-0-6-7\_vs\_3-5             & \textbf{0.9243 $\pm$ 0.0165}$^\dag$                                    & 0.0169 $\pm$ 0.0169 & 0.2106 $\pm$ 0.2724          & 0.4873 $\pm$ 0.3854          & 0.2074 $\pm$ 0.3146                                                    & 0.1794 $\pm$ 0.2752                                                    & 0.6440 $\pm$ 0.3504                                                   \\
	ecoli-0-6-7\_vs\_5               & \textbf{0.8926 $\pm$ 0.0147}$^\dag$                                    & 0.0139 $\pm$ 0.0139 & 0.0000 $\pm$ 0.0000          & 0.3887 $\pm$ 0.3800          & 0.2565 $\pm$ 0.3451                                                    & 0.2106 $\pm$ 0.3169                                                    & 0.3378 $\pm$ 0.3949                                                   \\
	ecoli3                           & 0.7112 $\pm$ 0.0142                                             & 0.0099 $\pm$ 0.0099 & 0.0000 $\pm$ 0.0000          & 0.5506 $\pm$ 0.4043          & 0.5991 $\pm$ 0.3587                                                    & 0.5730 $\pm$ 0.3270                                                    & \textbf{0.7712 $\pm$ 0.2738}                                          \\
	glass-0-1-2-3\_vs\_4-5-6         & \textbf{0.9877 $\pm$ 0.0084}$^\dag$                                    & 0.0879 $\pm$ 0.0879 & 0.1851 $\pm$ 0.3240          & 0.5906 $\pm$ 0.4080          & 0.1368 $\pm$ 0.2992                                                    & 0.0928 $\pm$ 0.1957                                                    & 0.6528 $\pm$ 0.4060                                                   \\
	glass-0-1-4-6\_vs\_2             & \textbf{0.9266 $\pm$ 0.0041}$^\dag$                                    & 0.0000 $\pm$ 0.0000 & 0.0000 $\pm$ 0.0000          & 0.0919 $\pm$ 0.1940          & 0.1256 $\pm$ 0.2057                                                    & 0.0416 $\pm$ 0.1316                                                    & 0.0000 $\pm$ 0.0000                                                   \\
	glass-0-1-5\_vs\_2               & \textbf{0.9837 $\pm$ 0.0044}$^\dag$                                    & 0.0000 $\pm$ 0.0000 & 0.0000 $\pm$ 0.0000          & 0.1440 $\pm$ 0.2413          & 0.1048 $\pm$ 0.2025                                                    & 0.0224 $\pm$ 0.0707                                                    & 0.0000 $\pm$ 0.0000                                                   \\
	glass-0-1-6\_vs\_2               & \textbf{0.7030 $\pm$ 0.0186}$^\dag$                                    & 0.0000 $\pm$ 0.0000 & 0.0000 $\pm$ 0.0000          & 0.0814 $\pm$ 0.1734          & 0.2035 $\pm$ 0.2158                                                    & 0.1666 $\pm$ 0.2261                                                    & 0.0000 $\pm$ 0.0000                                                   \\
	glass-0-1-6\_vs\_5               & \textbf{0.6785 $\pm$ 0.0058}                                    & 0.0066 $\pm$ 0.0066 & 0.1201 $\pm$ 0.2535          & 0.4598 $\pm$ 0.4051          & 0.3747 $\pm$ 0.4317                                                    & 0.5874 $\pm$ 0.3625                                                    & 0.0000 $\pm$ 0.0000                                                   \\
	glass-0-4\_vs\_5                 & \textbf{0.9837 $\pm$ 0.0083}                                    & 0.8943 $\pm$ 0.0860 & 0.1336 $\pm$ 0.2977          & 0.1665 $\pm$ 0.3558          & 0.0930 $\pm$ 0.2941                                                    & 0.0310 $\pm$ 0.0980                                                    & 0.2641 $\pm$ 0.4267                                                   \\
	glass-0-6\_vs\_5                 & \textbf{0.9486 $\pm$ 0.0174}$^\dag$                                    & 0.0187 $\pm$ 0.0187 & 0.0599 $\pm$ 0.1896          & 0.0000 $\pm$ 0.0000          & 0.2694 $\pm$ 0.3583                                                    & 0.2103 $\pm$ 0.3474                                                    & 0.4218 $\pm$ 0.3341                                                   \\
	glass0                           & \textbf{0.6785 $\pm$ 0.0362}$^\dag$                                    & 0.0327 $\pm$ 0.0327 & 0.0000 $\pm$ 0.0000          & 0.3342 $\pm$ 0.2762          & 0.1932 $\pm$ 0.2576                                                    & 0.0160 $\pm$ 0.0506                                                    & 0.2918 $\pm$ 0.3125                                                   \\
	glass1                           & \textbf{0.7641 $\pm$ 0.0139}$^\dag$                                    & 0.0151 $\pm$ 0.0151 & 0.0000 $\pm$ 0.0000          & 0.1163 $\pm$ 0.2453          & 0.1322 $\pm$ 0.2170                                                    & 0.1103 $\pm$ 0.2389                                                    & 0.1810 $\pm$ 0.2367                                                   \\
	glass2                           & \textbf{0.5105 $\pm$ 0.0636}$^\dag$                                   & 0.0000 $\pm$ 0.0000 & 0.0000 $\pm$ 0.0000          & 0.0967 $\pm$ 0.1908          & 0.1625 $\pm$ 0.2684                                                    & 0.0804 $\pm$ 0.1705                                                    & 0.0000 $\pm$ 0.0000                                                   \\
	glass4                           & \textbf{0.9486 $\pm$ 0.0261}                                    & 0.0237 $\pm$ 0.0237 & 0.0594 $\pm$ 0.1252          & 0.5909 $\pm$ 0.4081          & 0.5393 $\pm$ 0.4115                                                    & 0.5503 $\pm$ 0.3909                                                    & 0.1234 $\pm$ 0.2606                                                   \\
	glass5                           & \textbf{0.9951 $\pm$ 0.0019}$^\dag$                                    & 0.0017 $\pm$ 0.0017 & 0.0000 $\pm$ 0.0000          & 0.3332 $\pm$ 0.4302          & 0.4054 $\pm$ 0.3934                                                    & 0.4876 $\pm$ 0.3948                                                    & 0.0000 $\pm$ 0.0000                                                   \\
	glass6                           & \textbf{0.9354 $\pm$ 0.0644}                                    & 0.0624 $\pm$ 0.0624 & 0.1188 $\pm$ 0.2641          & 0.6041 $\pm$ 0.4170          & 0.5225 $\pm$ 0.4514                                                    & 0.6703 $\pm$ 0.2490                                                    & 0.6130 $\pm$ 0.4232                                                   \\
	haberman                         & \textbf{0.5105 $\pm$ 0.0224}                                    & 0.0248 $\pm$ 0.0248 & 0.0000 $\pm$ 0.0000          & 0.1400 $\pm$ 0.2295          & 0.0746 $\pm$ 0.1449                                                    & 0.2895 $\pm$ 0.2601                                                    & 0.0959 $\pm$ 0.2022                                                   \\
	iris0                            & \textbf{0.9450 $\pm$ 0.1918}                                    & 0.2006 $\pm$ 0.2006 & 0.0000 $\pm$ 0.0000          & 0.8882 $\pm$ 0.3143          & 0.1000 $\pm$ 0.3162                                                    & 0.1957 $\pm$ 0.4128                                                    & 0.1975 $\pm$ 0.4163                                                   \\
	\begin{tabular}[l]{@{}l@{}}led7digit-0-2-4-5-6-7\\ -8-9\_vs\_1\end{tabular} & \textbf{0.9951 $\pm$ 0.0543}                                    & 0.9731 $\pm$ 0.0438 & 0.7109 $\pm$ 0.0184          & 0.8248 $\pm$ 0.0062          & 0.8713 $\pm$ 0.1363                                                    & 0.8218 $\pm$ 0.1001                                                    & 0.8980 $\pm$ 0.0048                                                   \\
	new-thyroid1                     & \textbf{0.7379 $\pm$ 0.0787}$^\dag$                                    & 0.0784 $\pm$ 0.0784 & 0.0000 $\pm$ 0.0000          & 0.3671 $\pm$ 0.4113          & 0.1188 $\pm$ 0.2187                                                    & 0.0202 $\pm$ 0.0639                                                    & 0.1721 $\pm$ 0.1991                                                   \\
	newthyroid2                      & \textbf{0.8992 $\pm$ 0.0841}$^\dag$                                    & 0.0812 $\pm$ 0.0812 & 0.0000 $\pm$ 0.0000          & 0.2428 $\pm$ 0.2940          & 0.1434 $\pm$ 0.2648                                                    & 0.0000 $\pm$ 0.0000                                                    & 0.1773 $\pm$ 0.2409                                                   \\
	page-blocks-1-3\_vs\_4           & \textbf{0.9837 $\pm$ 0.0259}                                    & 0.0242 $\pm$ 0.0242 & 0.6504 $\pm$ 0.2320          & 0.5591 $\pm$ 0.3259          & 0.8324 $\pm$ 0.0776                                                    & 0.7323 $\pm$ 0.2629                                                    & 0.7211 $\pm$ 0.0211                                                   \\
	page-blocks0                     & \textbf{0.8649 $\pm$ 0.0944}                                    & 0.8595 $\pm$ 0.0123 & 0.8013 $\pm$ 0.0174          & 0.8593 $\pm$ 0.0150          & 0.8044 $\pm$ 0.0156                                                    & 0.6339 $\pm$ 0.2395                                                    & 0.8495 $\pm$ 0.0294                                                   \\
	pima                             & \textbf{0.9735 $\pm$ 0.0404}$^\dag$                                    & 0.0413 $\pm$ 0.0413 & 0.2468 $\pm$ 0.1941          & 0.5283 $\pm$ 0.2088          & 0.3099 $\pm$ 0.2907                                                    & 0.2580 $\pm$ 0.2628                                                    & 0.2581 $\pm$ 0.2782                                                   \\
	segment0                         & \textbf{0.8678 $\pm$ 0.0494}                                    & 0.0503 $\pm$ 0.0503 & 0.9261 $\pm$ 0.0164          & 0.6752 $\pm$ 0.4660          & 0.8240 $\pm$ 0.2898                                                    & 0.7582 $\pm$ 0.2444                                                    & 0.9358 $\pm$ 0.0141                                                   \\
	shuttle-c0-vs-c4                 & \textbf{0.9864 $\pm$ 0.0282}                                    & 0.9837 $\pm$ 0.0000 & 0.0000 $\pm$ 0.0000          & 0.8000 $\pm$ 0.4216          & 0.0189 $\pm$ 0.0598                                                    & 0.0378 $\pm$ 0.0797                                                    & 0.6984 $\pm$ 0.4819                                                   \\
	shuttle-c2-vs-c4                 & \textbf{0.7584 $\pm$ 0.0045}$^\dag$                                    & 0.0040 $\pm$ 0.0040 & 0.0775 $\pm$ 0.2449          & 0.4249 $\pm$ 0.3756          & 0.2677 $\pm$ 0.4328                                                    & 0.4859 $\pm$ 0.2866                                                    & 0.0000 $\pm$ 0.0000                                                   \\
	vehicle0                         & \textbf{0.9735 $\pm$ 0.0696}$^\dag$                                    & 0.0669 $\pm$ 0.0669 & 0.6686 $\pm$ 0.2367          & 0.6940 $\pm$ 0.2683          & 0.6598 $\pm$ 0.3107                                                    & 0.5708 $\pm$ 0.2897                                                    & 0.6381 $\pm$ 0.3452                                                   \\
	vowel0                           & 0.5136 $\pm$ 0.0231                                             & 0.0224 $\pm$ 0.0224 & 0.8880 $\pm$ 0.0780          & \textbf{0.9052 $\pm$ 0.0207} & 0.7299 $\pm$ 0.3872                                                    & 0.8465 $\pm$ 0.0189                                                    & 0.8968 $\pm$ 0.0448                                                   \\
	wisconsin                        & \textbf{0.9864 $\pm$ 0.1314}                                    & 0.1327 $\pm$ 0.1327 & 0.9694 $\pm$ 0.0035          & 0.8716 $\pm$ 0.3063          & 0.8761 $\pm$ 0.3084                                                    & 0.8702 $\pm$ 0.3058                                                    & 0.9748 $\pm$ 0.0150                                                   \\
	yeast-0-2-5-6\_vs\_3-7-8-9       & 0.7584 $\pm$ 0.0301                                             & 0.0341 $\pm$ 0.0341 & 0.3035 $\pm$ 0.2881          & 0.6602 $\pm$ 0.3277          & 0.6855 $\pm$ 0.2461                                                    & 0.7766 $\pm$ 0.0069                                                    & \textbf{0.8042 $\pm$ 0.1383}                                          \\
	yeast-0-2-5-7-9\_vs\_3-6-8       & \textbf{0.9545 $\pm$ 0.0486}                                    & 0.0489 $\pm$ 0.0489 & 0.5075 $\pm$ 0.2968          & 0.6991 $\pm$ 0.3477          & 0.5131 $\pm$ 0.3533                                                    & 0.5067 $\pm$ 0.3512                                                    & 0.8030 $\pm$ 0.1911                                                   \\
	yeast-0-3-5-9\_vs\_7-8           & \textbf{0.8822 $\pm$ 0.0164}$^\dag$                                    & 0.0180 $\pm$ 0.0180 & 0.0000 $\pm$ 0.0000          & 0.4785 $\pm$ 0.1819          & 0.3552 $\pm$ 0.3588                                                    & 0.2772 $\pm$ 0.3208                                                    & 0.5127 $\pm$ 0.1803                                                   \\
	yeast-0-5-6-7-9\_vs\_4           & \textbf{0.8944 $\pm$ 0.0144}                                    & 0.0161 $\pm$ 0.0161 & 0.0552 $\pm$ 0.1254          & 0.8093 $\pm$ 0.0301          & 0.8197 $\pm$ 0.0608                                                    & 0.6566 $\pm$ 0.2634                                                    & 0.7896 $\pm$ 0.2792                                                   \\
	yeast-1-2-8-9\_vs\_7             & \textbf{0.6975 $\pm$ 0.0003}                                    & 0.0004 $\pm$ 0.0004 & 0.0000 $\pm$ 0.0000          & 0.5120 $\pm$ 0.3539          & 0.6440 $\pm$ 0.2282                                                    & 0.4730 $\pm$ 0.2764                                                    & 0.0000 $\pm$ 0.0000                                                   \\
	yeast-1-4-5-8\_vs\_7             & \textbf{0.8101 $\pm$ 0.0031}$^\dag$                                    & 0.0000 $\pm$ 0.0000 & 0.0000 $\pm$ 0.0000          & 0.2794 $\pm$ 0.3122          & 0.5847 $\pm$ 0.2132                                                    & 0.3642 $\pm$ 0.2674                                                    & 0.0000 $\pm$ 0.0000                                                   \\
	yeast-1\_vs\_7                   & 0.6323 $\pm$ 0.0081                                             & 0.0086 $\pm$ 0.0086 & 0.0000 $\pm$ 0.0000          & 0.6678 $\pm$ 0.0673          & 0.6861 $\pm$ 0.0943                                                    & 0.5891 $\pm$ 0.2111                                                    & \textbf{0.7442 $\pm$ 0.2618}                                          \\
	yeast-2\_vs\_4                   & \textbf{0.8822 $\pm$ 0.0279}                                    & 0.8818 $\pm$ 0.0180 & 0.0225 $\pm$ 0.0713          & 0.8668 $\pm$ 0.0308          & 0.4358 $\pm$ 0.3818                                                    & 0.4821 $\pm$ 0.2760                                                    & 0.7102 $\pm$ 0.3744                                                   \\
	yeast-2\_vs\_8                   & \textbf{0.8944 $\pm$ 0.0301}$^\dag$                                    & 0.0303 $\pm$ 0.0303 & 0.0519 $\pm$ 0.1641          & 0.5792 $\pm$ 0.3053          & 0.2663 $\pm$ 0.2344                                                    & 0.2160 $\pm$ 0.2865                                                    & 0.5753 $\pm$ 0.2132                                                   \\
	yeast1                           & \textbf{0.6975 $\pm$ 0.0074}$^\dag$                                    & 0.0331 $\pm$ 0.0331 & 0.0454 $\pm$ 0.1049          & 0.2532 $\pm$ 0.3297          & 0.2979 $\pm$ 0.2633                                                    & 0.2359 $\pm$ 0.2170                                                    & 0.5126 $\pm$ 0.2635                                                   \\
	yeast3                           & \textbf{0.8101 $\pm$ 0.0174}                                    & 0.7992 $\pm$ 0.0238 & 0.0000 $\pm$ 0.0000          & 0.6761 $\pm$ 0.3563          & 0.5040 $\pm$ 0.4158                                                    & 0.4681 $\pm$ 0.3152                                                    & 0.3880 $\pm$ 0.3935                                                   \\
	yeast4                           & 0.6323 $\pm$ 0.0369                                             & 0.5062 $\pm$ 0.1069 & 0.5666 $\pm$ 0.4055          & 0.7744 $\pm$ 0.2721          & 0.8295 $\pm$ 0.2915                                                    & 0.8982 $\pm$ 0.0024                                                    & \textbf{0.9289 $\pm$ 0.0032}                                          \\
	yeast5                           & 0.8537 $\pm$ 0.0201                                             & 0.0099 $\pm$ 0.0099 & \textbf{0.9654 $\pm$ 0.0007} & 0.7719 $\pm$ 0.4068          & 0.7815 $\pm$ 0.3819                                                    & 0.9269 $\pm$ 0.0014                                                    & 0.8734 $\pm$ 0.3069\\
	\hline    
	Average Rank                                                     & \textbf{1.4310} & 5.8103 & 5.8534                                              & 3.4483                                               & 3.6207                                                              & 4.3879                                                              & 3.4483                                                      \\ 
	Win-lose-draw& - & 51-0-7 & 52-0-6 & 43-3-12 &	45-2-11    & 44-4-10 & 44-2-12    \\
	%Wilcoxon Signed-Rank Test & - & \textbf{3.50605E-11}	 & \textbf{8.91654E-11}	  & \textbf{7.31882E-10}	   & \textbf{5.45180E-10}	    & \textbf{5.19050E-10}	     & \textbf{8.20567E-09}	     \\	   
	Holm-Post hoc Test & - & \textbf{1.75303E-11}	 & \textbf{4.45971E-11}	  & \textbf{3.65941E-10}	   & \textbf{2.72630E-10}	    & \textbf{2.59525E-10}	     & \textbf{4.10284E-09}	     \\
	\hline                                              
\end{tabular}
\\$\dag$ indicates that the difference between the proposed algorithm and all other compared algorithm is statistically significant using pair-wised Wilcoxon rank sum test at the $5\%$ significance level.
\end{scriptsize}
\end{table*}

% Win-lose-draw
% Holm-Post hoc test

==> table/imbalance_benchmark_results_ranking_matrix.tex <==
\begin{table}[!h]
\centering
\caption{Comparison of the Average Ranking of Different Algorithms in Terms of Accuracy and G-Mean.}
\label{tab:imbalance_benchmark_result_ranking_matrix}
\begin{tiny}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\begin{tabular}[c]{@{}c@{}}Average \\ Ranking\end{tabular} & ECSDBN          & DBN    & \begin{tabular}[c]{@{}c@{}}DBN\\ -ADSN\end{tabular} & \begin{tabular}[c]{@{}c@{}}DBN\\ -SMOTE\end{tabular} & \begin{tabular}[c]{@{}c@{}}DBN\\ -SMOTE\\ -borderline1\end{tabular} & \begin{tabular}[c]{@{}c@{}}DBN\\ -SMOTE\\ -borderline2\end{tabular} & \begin{tabular}[c]{@{}c@{}}DBN\\ -SMOTE\\ -SVM\end{tabular} \\ \hline
Accuracy                                                   & \textbf{1.6466} & 1.8190 & 5.0690                                              & 4.8017                                               & 5.1034                                                              & 5.8448                                                              & 3.7155                                                      \\ \hline
G-mean                                                     & \textbf{1.4310} & 5.8103 & 5.8534                                              & 3.4483                                               & 3.6207                                                              & 4.3879                                                              & 3.4483                                                      \\ \hline
\end{tabular}
\end{tiny}
\end{table}
